NASIM: Revealing the low surface brightness Universe from legacy VISTA data

Near-infrared imaging is a powerful technique in observational astronomy, but the bright background, primarily from the Earth\'s atmosphere, makes the detection of faint features particularly challenging. To recover low surface brightness (LSB) structures in such data, we present NASIM (Near-infrared Automated low Surface brightness reduction In Maneage), a fully automated and reproducible data reduction pipeline optimised for VISTA/VIRCAM observations. NASIM builds on GNU Astronomy Utilities (Gnuastro) to effectively remove large-scale instrumental artefacts while preserving faint, diffuse emission. As a key science application, we focus on deep Ks-band observations of the Euclid Deep Field South (KEDFS), one of the deepest VISTA/VIRCAM datasets and a high-priority field for synergy with current and future facilities, including Euclid, JWST, LSST, Roman, Spitzer, and ALMA. With VIRCAM no longer operational, KEDFS now stands as a unique legacy dataset. We release selected tiles from the KEDFS survey and highlight science cases, including galaxy outskirts, LSB galaxies, and intracluster light, that demonstrate NASIM\'s ability to recover diffuse structures. A direct comparison with conventional VISTA data reduction pipelines demonstrates the advantages of NASIM in preserving diffuse emission without compromising compact source detection. All quantitative results presented in this paper are fully reproducible with Maneage (commit 4d32667).

==> project <==
#!/bin/sh
#
# High-level script to manage the project.
# Run './project --help' for a description of how to use it.
#
# Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
# Copyright (C) 2021-2023 Raul Infante-Sainz <infantesainz@gmail.com>
#
# This program is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.


# Basic settings
# --------------
# Stop the script if there are any errors.
set -e





# Default option values
jobs=0     # 0 is for the default for the 'configure.sh' script.
group=
debug=
host_cc=0
operation=
build_dir=
input_dir=
check_config=
make_targets=
software_dir=
clean_texdir=0
prepare_redo=0
highlightnew=0
all_highlevel=0
existing_conf=0
highlightnotes=0
scriptname="./project"





# Parse the options
# -----------------
#
# Separate command-line arguments from options. Then put the option value
# into the respective variable.
#
# Each option has two lines because we want to process both these formats:
# '--name=value' and '--name value'. The former (with '=') is a single
# command-line argument, so we just need to shift the counter by one. The
# latter (without '=') is two arguments, so we'll need two shifts.
#
# Note on the case strings: for every option, we need three lines: one when
# the option name and value are separate. Another when there is an equal
# between them, and finally one where the value is immediately after the
# short-format. This exact order is important. Otherwise, there will be a
# conflict between them.

print_help() {
    # Print the output.
    cat <<EOF
Usage: $scriptname configure [OPTIONS]
       $scriptname shell     [OPTIONS]
       $scriptname make      [OPTIONS]

Top-level script to manage the reproducible project. The high-level
operation is defined by the (mandatory) second argument:

  configure    - Configure project for this machine (e.g., build software).
  make         - Run the project (do analysis and build outputs).
  shell        - Execute the project's shell for interactive testing.

RECOMMENDATION: If this is the first time you are configuring this
template, please don't use the options and let the script explain each
parameter in full detail by simply running './project configure'.

Project 'make' special features.
  ./project make           Build the project on one thread
  ./project make -jN       Built the project in parallel on N threads.
  ./project make clean     Clean all files generated by 'make' (not software).
  ./project make texclean  Clean all files built by (La)TeX.
  ./project make distclean Clean everything (including compiled software).
  ./project make dist      Produce a LaTeX-ready-to-build distribution tarball
                           ('tar.gz') of the project. This is ready to be
                           uploaded to servers like 'arXiv.org'.
  ./project make dist-lzip Similar to 'dist', but compress to '.tar.lz'.
  ./project make dist-zip  Similar to 'dist', but compress to '.zip'.
  ./project make dist-software  Build a .tar.gz tarball containing all
                                software source tarballs necessary for the
                                project.

With the options below you can modify the default behavior.
Configure options:
  -b, --build-dir=STR      Top directory to build the project in.
  -e, --existing-conf      Use (possibly existing) local configuration.
      --host-cc            Use host system's C compiler, don't build GCC.
  -i, --input-dir=STR      Directory containing input datasets (optional).
  -s, --software-dir=STR   Directory containing necessary software tarballs.
      --check-config       During configuration, show what is being built.
      --clean-texdir       Remove possibly existing build-time subdirectories
                           under the project's 'tex/' directory (can happen
                           when source is from arXiv for example).
      --all-highlevel      Build all high-level software (for development).

Configure and Make options:
  -d, --debug[=FLAGS]      In configure: use -j1, no -k, and no Zenodo check.
                           In make: 'FLAGS' will be directly passed to 'make'.
  -g, --group=STR          Build and run with write permissions for a group.
  -j, --jobs=INT           Number of threads to build/run the software.
  -?, --help               Print this help list.

Make (analysis) options:
  -p, --prepare-redo       Re-do preparation (only done automatically once).

Make (final PDF) options:
      --refresh-bib        Force refresh the bibliography.
      --highlight-new      Highlight '\new' parts of text as green.
      --highlight-notes    Show '\tonote' regions as red text in PDF.

Mandatory or optional arguments to long options are also mandatory or optional
for any corresponding short options.

Maneage URL: https://maneage.org

Report bugs to mohammad@akhlaghi.org
EOF
}

on_off_option_error() {
    if [ "x$2" = x ]; then
        echo "$scriptname: '$1' doesn't take any values."
    else
        echo "$scriptname: '$1' (or '$2') doesn't take any values."
    fi
    exit 1
}

check_v() {
    if [ x"$2" = x ]; then
        echo "$scriptname: option '$1' requires an argument."
        echo "Try '$scriptname --help' for more information."
        exit 1;
    fi
}

func_operation_set() {
    if [ x$operation = x ]; then
        operation=$1
    else
        echo "Only one operation ('configure', 'make' or 'shell') may be given."
        exit 1
    fi
}

while [ $# -gt 0 ]
do
 case $1 in
  # Main operation.
  configure)    func_operation_set $1; shift;;
  make)         func_operation_set $1; shift;;
  shell)        func_operation_set $1; shift;;

  # Configure options:
  -b|--build-dir)        build_dir="$2";                                     check_v "$1" "$build_dir";    shift;shift;;
  -b=*|--build-dir=*)    build_dir="${1#*=}";                                check_v "$1" "$build_dir";    shift;;
  -b*)                   build_dir=$(echo    "$1" | sed -e's/-b//');         check_v "$1" "$build_dir";    shift;;
  -e|--existing-conf)    existing_conf=1;                                                                  shift;;
  -e*|--existing-conf=*) on_off_option_error --existing-conf -e;;
  --host-cc)             host_cc=1;                                                                        shift;;
  --host-cc=*)           on_off_option_error --host-cc;;
  -i|--input-dir)        input_dir="$2";                                     check_v "$1" "$input_dir";    shift;shift;;
  -i=*|--input-dir=*)    input_dir="${1#*=}";                                check_v "$1" "$input_dir";    shift;;
  -i*)                   input_dir=$(echo    "$1" | sed -e's/-i//');         check_v "$1" "$input_dir";    shift;;
  -s|--software-dir)     software_dir="$2";                                  check_v "$1" "$software_dir"; shift;shift;;
  -s=*|--software-dir=*) software_dir="${1#*=}";                             check_v "$1" "$software_dir"; shift;;
  -s*)                   software_dir=$(echo "$1" | sed -e's/-s//');         check_v "$1" "$software_dir"; shift;;
  --check-config)        check_config=1;                                                                   shift;;
  --check-config=*)      on_off_option_error --check-config;;
  --clean-texdir)        clean_texdir=1;                                                                   shift;;
  --clean-texdir=*)      on_off_option_error --clean-texdir;;
  --all-highlevel)       all_highlevel=1;                                                                  shift;;
  --all-highlevel=*)     on_off_option_error --all-highlevel;;

  # Configure and Make options:
  -g|--group)             group="$2";                            check_v group "$group";   shift;shift;;
  -g=*|--group=*)         group="${1#*=}";                       check_v group "$group";   shift;;
  -g*)                    group=$(echo   "$1" | sed -e's/-g//'); check_v group "$group";   shift;;
  -j|--jobs)              jobs="$2";                             check_v jobs  "$jobs";    shift;shift;;
  -j=*|--jobs=*)          jobs="${1#*=}";                        check_v jobs  "$jobs";    shift;;
  -j*)                    jobs=$(echo "$1" | sed -e's/-j//');    check_v jobs  "$jobs";    shift;;
  -'?'|--help)            print_help; exit 0;;
  -'?'*|--help=*)         on_off_option_error --help -?;;

  # Make options
  # ------------
  #
  # Note that Make's 'debug' can take values, but when called without any
  # value, it is like giving it a value of 'a'):
  --refresh-bib)          [ -f tex/src/references.tex ] && touch tex/src/references.tex;   shift;;
  --highlight-new)        highlightnew=1;                                                  shift;;
  --highlight-new=*)      on_off_option_error --highlight-new;;
  --highlight-notes)      highlightnotes=1;                                                shift;;
  --highlight-notes=*)    on_off_option_error --highlight-notes;;
  -d|--debug)             if [ x$operation = x ]; then
                              echo "Please set the operation before calling '--debug'"; exit 1
                          elif [ x$operation = xconfigure ]; then debug=a;   shift;
                          elif [ x$operation = xmake ]; then
                              if [ x"$2" = x ]; then echo "In make-mode, '--debug' needs a value"; exit 1
                              else debug="$2"; check_v debug "$debug"; shift;shift; fi
                          else
                              echo "Operation '$operation' not recognized, please use 'configure' or 'make'"
                          fi;;
  -d=*|--debug=*)         debug="${1#*=}";                       check_v debug "$debug";   shift;;
  -d*)                    debug=$(echo "$1" | sed -e's/-d//');   check_v debug "$debug";   shift;;
  -p|--prepare-redo)      prepare_redo=1;                                                  shift;;
  -p=*|--prepare-redo=*)  on_off_option_error --prepare-redo;                              shift;;

  # Unrecognized option:
  -*) echo "$scriptname: unknown option '$1'"; exit 1;;

  # Not an option, an argument (so its a Make target).
  *) make_targets="$make_targets $1"; shift;;
 esac
done





# Check configuration status
# --------------------------
if ! [ x$check_config = x ]; then
    # Find the color option to pass to 'ls'. Note that '--color' (for GNU
    # Coreutils 'ls') should be checked first because it also has '-G', but
    # for something else.
    if   ls --color 2> /dev/null > /dev/null; then coloropt="--color=auto"
    elif ls -G      2> /dev/null > /dev/null; then coloropt="-G"
    else                               coloropt=""
    fi

    # Print a notice to let the user know what is happening.
    cat <<EOF

This is an infinite loop that will print what software are being built at
every moment. It is actually a listing ('ls' command) of the temporary
directory where software source code are unpacked while they are being
built. If the project isn't being configured, the output (every second)
will either be empty (only a date) or a with an error about a non-existant
directory. This feature is thus only useful when the project's software are
being built.

EOF

    # Run the infinite loop. To be able to find the last built programs, we
    # need to put all the Python programs and high-level program into one
    # directory.
    checkdir=.local/version-info/.for-check-config
    while true; do

        # Make sure the '.build' directory has already been created.
        echo;
        echo "========================"
        if [ -d .build ]; then
            echo "$(date)    [[press CTRL-C to stop]]";
            echo "--- Currently being built:"
            if [ -d .build/software/build-tmp ]; then
                ls $coloropt .build/software/build-tmp || junk=1;
            fi

            # Make the temporary directory, delete its contents, then put new
            # links of all built software.
            if ! [ -d $checkdir ]; then mkdir $checkdir; fi
            rm -f $checkdir/*

            # Check if any programs exist in the given directory yet.
            printresults=0
            check=$(ls .local/version-info/python/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/python/*  $checkdir/
            fi
            check=$(ls .local/version-info/proglib/)
            if ! [ "x$check" = x ]; then
                printresults=1
                ln -s "$(pwd)"/.local/version-info/proglib/* $checkdir/
            fi

            # If something was actually found, then print them.
            if [ $printresults = 1 ]; then
                echo "--- Last 5 packages that were built:"

                # Then sort all the links based on the most recent dates of the
                # files they link to (with '-L').
                ls -Llt $checkdir  \
                    | awk '/^-/ && c++<5 {printf "[at %s] %s\n", $(NF-1), $NF}'
            fi
        else
            cat <<EOF
The connection to the build directory (.build) is not yet created.

If you have just ran './project configure', it should be created and will
be used in a few seconds to report the build status of various software.
If not, please run './project configure' (in another terminal) and you will
see the results shortly afterwards.
EOF
        fi
        echo "========================"

        # Wait for the next round of checks.
        sleep 1
    done
    exit 0
fi





# Basic group settings
# --------------------
if ! [ x$group = x ]; then

    # Check if group is usable.
    if ! sg "$group" "echo Group \'$group\' exists"; then
        echo "$scriptname: '$group' is not a usable group name on this system.";
        echo "(TIP: you can use the 'groups' command to see your groups)"
        exit 1
    fi

    # Set the group option for running Make.
    gopt="maneage_group_name=$group"
fi





# Error when configuration isn't run
configuration_necessary() {
    cat <<EOF

The project is either (1) not configured on this system, or (2) the
configuration wasn't successful.

(1) If it hasn't been configured at all, use the command below to configure
it (set a build directory and let it build its necessary software in it).

      $ ./project configure

(2) If it has been configured, but the configuration failed in a step, you
can re-configure it using your previous settings with the command
below. All successful steps will be skipped, allowing a fast completion.

      $ ./project configure -e

If there was a problem, please let us know by filling this online form:
      http://savannah.nongnu.org/support/?func=additem&group=reproduce

EOF
    exit 1
}





# Run operations in controlled environment
# ----------------------------------------
controlled_env() {

    # Get the full address of the build directory:
    bdir=`.local/bin/realpath .build`

    # Remove all existing environment variables (with 'env -i') and only
    # use some pre-defined environment variables, then build the project.
    envmake=".local/bin/env -i HOME=$bdir sys_rm=$(which rm) $gopt"
    envmake="$envmake highlightnew=$highlightnew"
    envmake="$envmake highlightnotes=$highlightnotes .local/bin/make"
    envmake="$envmake --no-builtin-rules --no-builtin-variables -f $1"
    if ! [ x"$debug" = x  ]; then envmake="$envmake --debug=$debug"; fi

    # Set the number of jobs. Note that for the 'configure.sh' script the
    # default value has to be 0, so the default is the maximum number of
    # threads. But here, the default value is 1.
    if ! [ x"$jobs"  = x0 ]; then envmake="$envmake -j$jobs";  fi

    # Run the project
    if [ x"$group" = x ]; then
        $envmake $make_targets
    else
        # Set the group and permission flags.
        sg "$group" "umask $perms && $envmake $make_targets"
    fi
}





# Do requested operation
# ----------------------
perms="u+r,u+w,g+r,g+w,o-r,o-w,o-x"
configscript=./reproduce/software/shell/configure.sh
case $operation in

    # Build the project's software.
    configure)

        # Set executable flags
        # --------------------
        #
        # In some scenarios (for example when using a tarball from arXiv),
        # it may happen that the host server has removed the executable
        # flags of all the files. In 'README.md' we instruct the readers on
        # setting the executable flag of this script. But we don't want the
        # user to have to worry about any other file that needs an
        # executable flag.
        #
        # Basically, all the project shell scripts need executable flags so
        # to make sure they have them, we are activating the executable
        # flags by default here every time './project configure' is run. If
        # any other file in your project needs such flags, add them here.
        chmod +x reproduce/software/shell/* reproduce/software/config/*.sh \
              reproduce/analysis/bash/*

        # If the user requested, clean the TeX directory from the extra
        # (to-be-built) directories that may already be there (and will not
        # allow the configuration to complete).
        if [ x"$clean_texdir" = x1 ]; then
            rm -rf tex/build tex/tikz
        fi

        # Variables to pass to the configuration script.
        export jobs=$jobs
        export debug=$debug
        export host_cc=$host_cc
        export build_dir=$build_dir
        export input_dir=$input_dir
        export scriptname=$scriptname
        export maneage_group_name=$group
        export software_dir=$software_dir
        export existing_conf=$existing_conf
        export all_highlevel=$all_highlevel

        # Run the configuration script
        if [ x"$group" = x ]; then
            $configscript
        else
            # Set the group and permission flags.
            sg "$group" "umask $perms && $configscript"

            # Set the group writing permission for everything in the
            # installed software directory. The common build process sets
            # the writing permissions of the installed programs/libraries
            # to '755'. So group members can't write over a file. This
            # creates problems when another group member wants to update
            # the software for example. We thus need to manually add the
            # group writing flag to all installed software files.
            echo "Enabling group writing permission on all installed software..."
            .local/bin/chmod -R g+w .local/;
        fi
        ;;





    # Batch execution of the project.
    make)

        # Make sure the configure script has been completed properly
        # ('configuration-done.txt' exists).
        if ! [ -f .build/software/configuration-done.txt ]; then
            configuration_necessary
        fi

        # Add extra preparation step for completing of 'INPUTS.conf'.
        if ! [ -f .build/software/listurl-done.mk ] \
                || [ x"$prepare_redo" = x1 ]; then
            controlled_env reproduce/analysis/make/top-listurl.mk
        fi

        # Run data preparation phase (optionally build Makefiles with
        # special values for optimizing the main 'top-make.mk'). But note
        # that data preparation is only done automatically the first time
        # the project is built (when '.build/software/preparation-2-done.mk'
        # doesn't yet exist). After that, if the user wants to re-do the
        # preparation they have to use the '--prepare-redo' option.
        if ! [ -f .build/software/ingest-done.mk ] \
                || [ x"$prepare_redo" = x1 ]; then
            controlled_env reproduce/analysis/make/top-ingest.mk
        fi

        # Run the actual project.
        controlled_env reproduce/analysis/make/top-make.mk
        ;;


    shell)

        # Make sure the configure script has been completed properly
        # ('configuration-done.txt' exists).
        if ! [ -f .build/software/configuration-done.txt ]; then
            configuration_necessary
        fi

        # Run the project's own shell without inheriting any environment
        # from the host. The 'TERM' environment variable is necessary for
        # tools like some text editors.
        bdir=`.local/bin/realpath .build`
        instdir="$bdir"/software/installed
        bindir="$bdir"/software/installed/bin
        rcfile=$(pwd)/reproduce/software/shell/bashrc.sh
        .local/bin/env -i \
                       HOME="$bdir" \
                       TERM="$TERM" \
                       PATH="$bindir" \
                       CCACHE_DISABLE=1 \
                       PROJECT_STATUS=shell \
                       SHELL="$bindir"/bash \
                       COLORTERM="$COLORTERM" \
                       PROJECT_RCFILE="$rcfile" \
                       LDFLAGS=-L"$instdir"/lib \
                       CPPFLAGS=-I"$instdir"/include \
                       LD_LIBRARY_PATH="$instdir"/lib \
                       OMPI_MCA_plm_rsh_agent=/bin/false \
                       PYTHONPATH="$instdir"/lib/python/site-packages \
                       PYTHONPATH3="$instdir"/lib/python/site-packages \
                       PS1="[\[\033[01;35m\]maneage@\h \W\[\033[32m\]\[\033[00m\]]$ " \
                       "$bindir"/bash --noprofile --rcfile "$rcfile"
        ;;


    # Operation not specified.
    *)
        cat <<EOF

No operation defined!

Please run with '--help' for more information.
(TIP: available operations are: 'configure', 'make', or 'shell').

EOF
        exit 1
        ;;
esac


==> reproduce/analysis/bash/download-multi-try <==
#!/bin/sh
#
# Attempt downloading multiple times before crashing whole project. From
# the top project directory (for the shebang above), this script must be
# run like this:
#
#   $ /path/to/download-multi-try downloader lockfile input-url downloaded-name
#
# NOTE: The 'downloader' must contain the option to specify the output name
# in its end. For example "wget -O". Any other option can also be placed in
# the middle.
#
# Due to temporary network problems, a download may fail suddenly, but
# succeed in a second try a few seconds later. Without this script that
# temporary glitch in the network will permanently crash the project and
# it can't continue. The job of this script is to be patient and try the
# download multiple times before crashing the whole project.
#
# LOCK FILE: Since there is usually only one network port to the outside
# world, downloading is done much faster in serial, not in parallel. But
# the project's processing may be done in parallel (with multiple threads
# needing to download different files at the same time). Therefore, this
# script uses the 'flock' program to only do one download at a time. To
# benefit from it, any call to this script must be given the same lock
# file. If your system has multiple ports to the internet, or for any
# reason, you don't want to use a lock file, set the 'lockfile' name to
# 'nolock'.
#
# Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This program is free software: you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation, either version 3 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program.  If not, see <http://www.gnu.org/licenses/>.





# Script settings
# ---------------
# Stop the script if there are any errors.
set -e





# Input arguments and necessary sanity checks. Note that the 5th argument
# (backup servers) isn't mandatory.
inurl="$3"
outname="$4"
lockfile="$2"
downloader="$1"
backupservers="$5"
if [ "x$downloader" = x ]; then
    echo "$0: downloader (first argument) not given."; exit 1;
fi
if [ "x$lockfile" = x ]; then
    echo "$0: lock file (second argument) not given."; exit 1;
fi
if [ "x$inurl" = x ]; then
    echo "$0: full input URL (third argument) not given."; exit 1;
fi
if [ "x$outname" = x ]; then
    echo "$0: output name (fourth argument) not given."; exit 1;
fi





# Separate the actual filename, to possibly use backup server.
urlfile=$(echo "$inurl" | awk -F "/" '{print $NF}')





# Try downloading multiple times before crashing.
counter=0
maxcounter=10
while [ ! -f "$outname" ]; do

    # Increment the counter.
    counter=$(echo $counter | awk '{print $1+1}')

    # If we have passed a maximum number of trials, just exit with
    # a failed code.
    reachedmax=$(echo $counter \
         | awk '{if($1>'$maxcounter') print "yes"; else print "no";}')
    if [ x$reachedmax = xyes ]; then
        echo ""
	echo "Failed $maxcounter download attempts: $outname"
        echo ""
	exit 1
    fi

    # If this isn't the first attempt print a notice and wait a little for
    # the next trail.
    if [ x$counter = x1 ]; then
        just_a_place_holder=1
    else
        tstep=$(echo $counter | awk '{print $1*5}')
        echo "Download trial $counter for '$outname' in $tstep seconds."
        sleep $tstep
    fi

    # Attempt downloading the file. Note that the 'downloader' ends with
    # the respective option to specify the output name. For example "wget
    # -O" (so 'outname', that comes after it) will be the name of the
    # downloaded file.
    if [ x"$lockfile" = xnolock ]; then
        if ! $downloader $outname $inurl; then rm -f $outname; fi
    else
        # Try downloading from the requested URL.
        flock "$lockfile" sh -c \
              "if ! $downloader $outname \"$inurl\"; then rm -f $outname; fi"
    fi

    # If the download failed, try the backup server(s).
    if [ ! -f "$outname" ]; then
        if [ x"$backupservers" != x ]; then
            for bs in $backupservers; do

                # Use this backup server.
                if [ x"$lockfile" = xnolock ]; then
                    if ! $downloader $outname $bs/$urlfile; then rm -f $outname; fi
                else
                    flock "$lockfile" sh -c \
                          "if ! $downloader $outname $bs/$urlfile; then rm -f $outname; fi"
                fi

                # If the file was downloaded, break out of the loop that
                # parses over the backup servers.
                if [ -f "$outname" ]; then break; fi
            done
        fi
    fi
done





# Return successfully
exit 0


==> reproduce/software/bibtex/astrometrynet.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astrometrynet,
       author = {{Lang}, Dustin and {Hogg}, David W. and {Mierle}, Keir and {Blanton}, Michael and {Roweis}, Sam},
        title = "{Astrometry.net: Blind Astrometric Calibration of Arbitrary Astronomical Images}",
      journal = {AJ},
     keywords = {astrometry, catalogs, instrumentation: miscellaneous, methods: data analysis, methods: statistical, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = may,
       volume = {139},
       number = {5},
        pages = {1782-1800},
          doi = {10.1088/0004-6256/139/5/1782},
archivePrefix = {arXiv},
       eprint = {0910.2233},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....139.1782L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/astropy.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astropy2018,
   author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H o}cz}, B.~M. and
	{G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and
	{Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and
	{Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and
	{P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and
	{Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and
	{Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and
	{Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and
	{Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and
	{Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and
	{Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'{\i}}guez}, J.~L. and
	{Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and
	{Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and
	{Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and
	{Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and
	{Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and
	{Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and
	{Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and
	{Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and
	{Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and
	{Ivezi{\'c}}, {\v Z}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and
	{Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and
	{Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and
	{Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and
	{Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and
	{Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and
	{Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and
	{Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and
	{Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and
	{Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and
	{Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and
	{Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and
	{Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and
	{Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and
	{Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and
	{Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and
	{van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and
	{Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and
	{Zabalza}, V. and {Astropy Contributors}},
    title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
  journal = {AJ},
archivePrefix = "arXiv",
   eprint = {1801.02634},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems },
     year = 2018,
    month = sep,
   volume = 156,
      eid = {123},
    pages = {123},
      doi = {10.3847/1538-3881/aabc4f},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{astropy2013,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and
	{Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and
	{Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and
	{Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and
	{Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and
	{Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and
	{Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and
	{Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and
	{Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and
	{Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and
	{Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and
	{Servillat}, M. and {Streicher}, O.},
    title = "{Astropy: A community Python package for astronomy}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2013A\%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/corner.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{corner,
       author = {{Foreman-Mackey}, Daniel},
        title = "{corner.py: Scatterplot matrices in Python}",
      journal = {JOSS},
         year = "2016",
        month = "Jun",
       volume = {1},
        pages = {24},
          doi = {10.21105/joss.00024},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JOSS....1...24F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/cython.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{cython2011,
       author = {{Behnel}, Stefan and {Bradshaw}, Robert and {Citro}, Craig and {Dalcin}, Lisandro and {Seljebotn}, Dag Sverre and {Smith}, Kurt},
        title = "{Cython: The Best of Both Worlds}",
      journal = {Computing in Science and Engineering},
         year = 2011,
        month = mar,
       volume = {13},
       number = {2},
        pages = {31-39},
          doi = {10.1109/MCSE.2010.118},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011CSE....13b..31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/fftw.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{fftw,
   author = {M. {Frigo} and S. G. {Johnson}},
  journal = {IEEE Proc.},
    title = {The Design and Implementation of FFTW3},
     year = {2005},
   volume = {93},
   number = {2},
    pages = {216-231},
      doi = {10.1109/JPROC.2004.840301},
     ISSN = {0018-9219},
    month = {Feb},
}


==> reproduce/software/bibtex/galsim.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{galsim,
       author = {{Rowe}, B.~T.~P. and {Jarvis}, M. and {Mandelbaum}, R. and
         {Bernstein}, G.~M. and {Bosch}, J. and {Simet}, M. and {Meyers}, J.~E. and
         {Kacprzak}, T. and {Nakajima}, R. and {Zuntz}, J. and {Miyatake}, H. and
         {Dietrich}, J.~P. and {Armstrong}, R. and {Melchior}, P. and
         {Gill}, M.~S.~S.},
        title = "{GALSIM: The modular galaxy image simulation toolkit}",
      journal = {Astron.Comput.},
     keywords = {Methods: data analysis, Techniques: image processing, Gravitational lensing, Cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, 85-04},
         year = "2015",
        month = "Apr",
       volume = {10},
        pages = {121-150},
          doi = {10.1016/j.ascom.2015.02.002},
archivePrefix = {arXiv},
       eprint = {1407.7676},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&C....10..121R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/gnuastro.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{gnuastro,
       author = {{Akhlaghi}, Mohammad and {Ichikawa}, Takashi},
        title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
      journal = {ApJS},
     keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = sep,
       volume = {220},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.1088/0067-0049/220/1/1},
archivePrefix = {arXiv},
       eprint = {1505.01664},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/healpix.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{healpix,
       author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and {Wandelt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and {Bartelmann}, M.},
        title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
      journal = {ApJ},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical, Astrophysics},
         year = 2005,
        month = apr,
       volume = {622},
       number = {2},
        pages = {759-771},
          doi = {10.1086/427976},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409513},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622..759G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/imfit.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{imfit2015,
       author = {{Erwin}, Peter},
        title = "{IMFIT: A Fast, Flexible New Program for Astronomical Image Fitting}",
      journal = {ApJ},
     keywords = {galaxies: bulges, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = feb,
       volume = {799},
       number = {2},
          eid = {226},
        pages = {226},
          doi = {10.1088/0004-637X/799/2/226},
archivePrefix = {arXiv},
       eprint = {1408.1097},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..226E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/matplotlib.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{matplotlib2007,
       author = {{Hunter}, John D.},
        title = "{Matplotlib: A 2D Graphics Environment}",
      journal = {CiSE},
     keywords = {Python, Scripting languages, Application development, Scientific programming},
         year = 2007,
        month = may,
       volume = {9},
       number = {3},
        pages = {90-95},
          doi = {10.1109/MCSE.2007.55},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007CSE.....9...90H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/missfits.tex <==
%% Copyright (C) 2020-2023 Surena Fatemi <surena.fatemi@ipm.ir>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{missfits,
       author = {{Marmo}, C. and {Bertin}, E.},
        title = "{MissFITS and WeightWatcher: Two Optimised Tools for Managing FITS Data.}",
      journal = {ASPC},
         year = 2008,
       volume = {394},
       series = {Astronomical Society of the Pacific Conference Series},
        pages = {619},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ASPC..394..619M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/mpi4py.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{mpi4py2011,
       author = {{Dalcin}, Lisandro D. and {Paz}, Rodrigo R. and {Kler}, Pablo A. and {Cosimo}, Alejandro},
        title = "{Parallel distributed computing using Python}",
      journal = {Advances in Water Resources},
         year = 2011,
        month = sep,
       volume = {34},
       number = {9},
        pages = {1124-1139},
          doi = {10.1016/j.advwatres.2011.04.013},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AdWR...34.1124D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/numpy.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{numpy2020,
       author = {{Harris}, Charles R. and {Millman}, K. Jarrod and {van der Walt}, St{\'e}fan J. and {Gommers}, Ralf and {Virtanen}, Pauli and {Cournapeau}, David and {Wieser}, Eric and {Taylor}, Julian and {Berg}, Sebastian and {Smith}, Nathaniel J. and {Kern}, Robert and {Picus}, Matti and {Hoyer}, Stephan and {van Kerkwijk}, Marten H. and {Brett}, Matthew and {Haldane}, Allan and {del R{\'\i}o}, Jaime Fern{\'a}ndez and {Wiebe}, Mark and {Peterson}, Pearu and {G{\'e}rard-Marchant}, Pierre and {Sheppard}, Kevin and {Reddy}, Tyler and {Weckesser}, Warren and {Abbasi}, Hameer and {Gohlke}, Christoph and {Oliphant}, Travis E.},
        title = "{Array programming with NumPy}",
      journal = {Nature},
     keywords = {Computer Science - Mathematical Software, Statistics - Computation},
         year = 2020,
        month = sep,
       volume = {585},
       number = {7825},
        pages = {357-362},
          doi = {10.1038/s41586-020-2649-2},
archivePrefix = {arXiv},
       eprint = {2006.10256},
 primaryClass = {cs.MS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020Natur.585..357H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/r-cran.tex <==
%% Copyright (C) 2022-2023 Boud Roukema <boud@cosmo.torun.pl>
%% Copyright (C) 2022-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{RIhakaGentleman1996,
      author = {{Ihaka}, Ross and {Gentleman}, Robert},
       title = "{R: A language for data analysis and graphics}",
     journal = {J.Comput.Graph.Stat.},
        year = {1996},
      volume = {5},
      number = {3},
       pages = {299-314},
         DOI = {10.1080/10618600.1996.10474713},
        ISSN = {10618600},
}


==> reproduce/software/bibtex/scamp.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scamp,
   author = {{Bertin}, E.},
    title = "{Automatic Astrometric and Photometric Calibration with SCAMP}",
     year = 2006,
   journal= {ASPConf},
   volume = 351,
    month = jul,
    pages = {112},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..351..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/scipy.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scipy2020,
       author = {{Virtanen}, Pauli and {Gommers}, Ralf and {Oliphant}, Travis E. and {Haberland}, Matt and {Reddy}, Tyler and {Cournapeau}, David and {Burovski}, Evgeni and {Peterson}, Pearu and {Weckesser}, Warren and {Bright}, Jonathan and {van der Walt}, St{\'e}fan J. and {Brett}, Matthew and {Wilson}, Joshua and {Millman}, K. Jarrod and {Mayorov}, Nikolay and {Nelson}, Andrew R.~J. and {Jones}, Eric and {Kern}, Robert and {Larson}, Eric and {Carey}, C.~J. and {Polat}, {\.I}lhan and {Feng}, Yu and {Moore}, Eric W. and {VanderPlas}, Jake and {Laxalde}, Denis and {Perktold}, Josef and {Cimrman}, Robert and {Henriksen}, Ian and {Quintero}, E.~A. and {Harris}, Charles R. and {Archibald}, Anne M. and {Ribeiro}, Ant{\^o}nio H. and {Pedregosa}, Fabian and {van Mulbregt}, Paul and {SciPy 1. 0 Contributors}},
        title = "{SciPy 1.0: fundamental algorithms for scientific computing in Python}",
      journal = {Nature Methods},
     keywords = {Computer Science - Mathematical Software, Computer Science - Data Structures and Algorithms, Computer Science - Software Engineering, Physics - Computational Physics},
         year = 2020,
        month = feb,
       volume = {17},
        pages = {261-272},
          doi = {10.1038/s41592-019-0686-2},
archivePrefix = {arXiv},
       eprint = {1907.10121},
 primaryClass = {cs.MS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NatMe..17..261V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sextractor.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sextractor,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {A\&AS},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = 1996,
        month = jun,
       volume = {117},
        pages = {393-404},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sip_tpv.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sip-tpv,
   author = {{Shupe}, D.~L. and {Laher}, R.~R. and {Storrie-Lombardi}, L. and
	{Surace}, J. and {Grillmair}, C. and {Levitan}, D. and {Sesar}, B.
	},
    title = "{More flexibility in representing geometric distortion in astronomical images}",
     year = 2012,
   journal = {SPIE},
   volume = 8451,
    month = sep,
      eid = {84511M},
    pages = {84511M},
      doi = {10.1117/12.925460},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2012SPIE.8451E..1MS},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/swarp.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{swarp,
   author = {{Bertin}, E. and {Mellier}, Y. and {Radovich}, M. and {Missonnier}, G. and
    {Didelon}, P. and {Morin}, B.},
  journal = {ASPConf},
    title = "{The TERAPIX Pipeline}",
     year = {2002},
   volume = {281},
    pages = {228},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2002ASPC..281..228B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sympy.tex <==
%% Copyright (C) 2019-2023 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@article{sympy,
 title = {SymPy: symbolic computing in Python},
 author = {Meurer, Aaron and Smith, Christopher P. and Paprocki, Mateusz and \v{C}ert\'{i}k, Ond\v{r}ej and Kirpichev, Sergey B. and Rocklin, Matthew and Kumar, AMiT and Ivanov, Sergiu and Moore, Jason K. and Singh, Sartaj and Rathnayake, Thilina and Vig, Sean and Granger, Brian E. and Muller, Richard P. and Bonazzi, Francesco and Gupta, Harsh and Vats, Shivam and Johansson, Fredrik and Pedregosa, Fabian and Curry, Matthew J. and Terrel, Andy R. and Rou\v{c}ka, \v{S}t\v{e}p\'{a}n and Saboo, Ashutosh and Fernando, Isuru and Kulal, Sumith and Cimrman, Robert and Scopatz, Anthony},
 year = 2017,
 month = jan,
 keywords = {Python, Computer algebra system, Symbolics},
 volume = 3,
 pages = {103},
 journal = {PeerJ CompSci},
 issn = {2376-5992},
 url = {https://doi.org/10.7717/peerj-cs.103},
 doi = {10.7717/peerj-cs.103}
}


==> reproduce/software/bibtex/tides.tex <==
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{tides,
   author = {{Abad}, A. and {Barrio}, R. and {Belsa}, F. and {Rodriguez}, M},
    title = "{Algorithm 924: TIDES, a Taylor Series Integrator for Differential EquationS}",
  journal = {ACM TOMS},
     year = 2012,
    month = nov,
   volume = 39,
      eid = {5},
    pages = {1-28},
      doi = {10.1145/2382585.2382590},
 keywords = {Taylor series method, automatic differentiation, high precision, numerical integration of ODEs, variational equations},
}


==> reproduce/software/shell/git-post-checkout <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). We have just changed the name of the 'MSFILE' and also
# set special characters for the installation location of meta-store so our
# own installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.


# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Delete all temporary files
find @TOP_PROJECT_DIR@/ -name "*~" -type f -delete

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Run metastore.
exit_on_fail \
       $MSBIN -a -m -e -E -q -O @USER@ -G @GROUP@ -f "$MSFILE"

# Return with a success code (0).
exit 0


==> reproduce/software/shell/git-pre-commit <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the 'metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# WARNING:
#
# If the commit is aborted (e.g. by not entering any synopsis),
# then updated metastore file (.metadata by default) is not reverted,
# so its new version remains in the index.
# To undo any changes in metastore file written since HEAD commit,
# you may want to reset and checkout HEAD version of the file:
#
#     git reset HEAD -- .metadata
#     git checkout HEAD -- .metadata
#
# This script is taken from the 'examples/hooks/pre-commit' file of the
# 'metastore' package (installed within the project, with an MIT license
# for copyright). Here, the name of the 'MSFILE' and also set special
# characters for the installation location of meta-store so our own
# installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.

# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Run metastore.
exit_on_fail \
	$MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"

# If it's first metastore commit, store again to include $MSFILE in $MSFILE.
if ! git-ls-tree --name-only HEAD 2>/dev/null | grep -Fqx "$MSFILE"; then
	exit_on_fail \
	        $MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"
fi

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Add the metadata file to the Git repository.
exit_on_fail \
	git-add "$MSFILE"

# Return with a success code (0).
exit 0


==> tex/src/journal-macros.tex <==
%% Extracted from: https://ui.adsabs.harvard.edu/help/actions/journal-macros
%% Extracted at 2022-04-12

\newcommand{\aj}{AJ}                   % Astronomical Journal
\newcommand{\actaa}{Acta Astron.}      % Acta Astronomica
\newcommand{\araa}{ARA\&A}             % Annual Review of Astron and Astrophys
\newcommand{\apj}{ApJ}                 % Astrophysical Journal
\newcommand{\apjl}{ApJ}                % Astrophysical Journal, Letters
\newcommand{\apjs}{ApJS}               % Astrophysical Journal, Supplement
\newcommand{\ao}{Appl.~Opt.}           % Applied Optics
\newcommand{\apss}{Ap\&SS}             % Astrophysics and Space Science
\newcommand{\aap}{A\&A}                % Astronomy and Astrophysics
\newcommand{\aapr}{A\&A~Rev.}          % Astronomy and Astrophysics Reviews
\newcommand{\aaps}{A\&AS}              % Astronomy and Astrophysics, Supplement
\newcommand{\azh}{AZh}                 % Astronomicheskii Zhurnal
\newcommand{\baas}{BAAS}               % Bulletin of the AAS
\newcommand{\bac}{Bull. astr. Inst. Czechosl.}
                % Bulletin of the Astronomical Institutes of Czechoslovakia
\newcommand{\caa}{Chinese Astron. Astrophys.}
                % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{Chinese J. Astron. Astrophys.}
                % Chinese Journal of Astronomy and Astrophysics
\newcommand{\icarus}{Icarus}           % Icarus
\newcommand{\jcap}{J. Cosmology Astropart. Phys.}
                % Journal of Cosmology and Astroparticle Physics
\newcommand{\jrasc}{JRASC}             % Journal of the RAS of Canada
\newcommand{\memras}{MmRAS}            % Memoirs of the RAS
\newcommand{\mnras}{MNRAS}             % Monthly Notices of the RAS
\newcommand{\na}{New A}                % New Astronomy
\newcommand{\nar}{New A Rev.}          % New Astronomy Review
\newcommand{\pra}{Phys.~Rev.~A}        % Physical Review A: General Physics
\newcommand{\prb}{Phys.~Rev.~B}        % Physical Review B: Solid State
\newcommand{\prc}{Phys.~Rev.~C}        % Physical Review C
\newcommand{\prd}{Phys.~Rev.~D}        % Physical Review D
\newcommand{\pre}{Phys.~Rev.~E}        % Physical Review E
\newcommand{\prl}{Phys.~Rev.~Lett.}    % Physical Review Letters
\newcommand{\pasa}{PASA}               % Publications of the Astron. Soc. of Australia
\newcommand{\pasp}{PASP}               % Publications of the ASP
\newcommand{\pasj}{PASJ}               % Publications of the ASJ
\newcommand{\rmxaa}{Rev. Mexicana Astron. Astrofis.}%
                % Revista Mexicana de Astronomia y Astrofisica
\newcommand{\qjras}{QJRAS}             % Quarterly Journal of the RAS
\newcommand{\skytel}{S\&T}             % Sky and Telescope
\newcommand{\solphys}{Sol.~Phys.}      % Solar Physics
\newcommand{\sovast}{Soviet~Ast.}      % Soviet Astronomy
\newcommand{\ssr}{Space~Sci.~Rev.}     % Space Science Reviews
\newcommand{\zap}{ZAp}                 % Zeitschrift fuer Astrophysik
\newcommand{\nat}{Nature}              % Nature
\newcommand{\iaucirc}{IAU~Circ.}       % IAU Cirulars
\newcommand{\aplett}{Astrophys.~Lett.} % Astrophysics Letters
\newcommand{\apspr}{Astrophys.~Space~Phys.~Res.}
                % Astrophysics Space Physics Research
\newcommand{\bain}{Bull.~Astron.~Inst.~Netherlands}
                % Bulletin Astronomical Institute of the Netherlands
\newcommand{\fcp}{Fund.~Cosmic~Phys.}  % Fundamental Cosmic Physics
\newcommand{\gca}{Geochim.~Cosmochim.~Acta}   % Geochimica Cosmochimica Acta
\newcommand{\grl}{Geophys.~Res.~Lett.} % Geophysics Research Letters
\newcommand{\jcp}{J.~Chem.~Phys.}      % Journal of Chemical Physics
\newcommand{\jgr}{J.~Geophys.~Res.}    % Journal of Geophysics Research
\newcommand{\jqsrt}{J.~Quant.~Spec.~Radiat.~Transf.}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\newcommand{\memsai}{Mem.~Soc.~Astron.~Italiana}
                % Mem. Societa Astronomica Italiana
\newcommand{\nphysa}{Nucl.~Phys.~A}   % Nuclear Physics A
\newcommand{\physrep}{Phys.~Rep.}   % Physics Reports
\newcommand{\physscr}{Phys.~Scr}   % Physica Scripta
\newcommand{\planss}{Planet.~Space~Sci.}   % Planetary Space Science
\newcommand{\procspie}{Proc.~SPIE}   % Proceedings of the SPIE

\newcommand{\astap}{\aap}
\newcommand{\apjlett}{\apjl}
\newcommand{\apjsupp}{\apjs}
\newcommand{\applopt}{\ao}


==> tex/src/preamble-biblatex.tex <==
%% Biblatex settings.
%%
%% Settings necessary to make the bibliography with Biblatex. Keeping all
%% BibLaTeX settings in a separate preamble was done in the spirit of
%% modularity to 1) easily managable, 2) If a similar BibLaTeX
%% configuration is necessary in another LaTeX compilation, this file can
%% just be copied there and used.
%%
%% USAGE:
%%  - 'tex/src/references.tex': the file containing Bibtex source of each
%%     reference. The file suffix doesn't have to be '.bib'. This naming
%%     helps in clearly identifying the files and avoiding places that
%%     complain about '.bib' files.
%
%% Copyright (C) 2018-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%
%% This file is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the
%% Free Software Foundation, either version 3 of the License, or (at your
%% option) any later version.
%
%% This file is distributed in the hope that it will be useful, but WITHOUT
%% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General Public License
%% for more details.
%
%% You should have received a copy of the GNU General Public License along
%% with this file.  If not, see <http://www.gnu.org/licenses/>.





%% For clarifing of the name of journals based on NASA website.
\input{tex/src/journal-macros.tex}





%% To break up highlighted text (for example texttt when some it is on the
%% line break) and also to no underline emphasized words (like journal
%% titles in the references).
\usepackage[normalem]{ulem}





%% For quotation signs (sometimes used by BibLaTeX)
\usepackage{csquotes}





%% To define colors
\usepackage{xcolor}





% Basic BibLaTeX settings
\usepackage[
    doi=false,
    url=false,
    dashed=false,
    eprint=false,
    maxbibnames=2,
    minbibnames=1,
    hyperref=true,
    maxcitenames=2,
    mincitenames=1,
    giveninits=true,
    style=authoryear,
    uniquelist=false,
    backend=biber,natbib]{biblatex}
\DeclareFieldFormat[article]{pages}{#1}
\DeclareFieldFormat{pages}{\mkfirstpage[{\mkpageprefix[bookpagination]}]{#1}}
\addbibresource{tex/src/references.tex}
\addbibresource{tex/build/macros/dependencies-bib.tex}
\renewbibmacro{in:}{}
\AtEveryBibitem{\clearfield{month}}
\renewcommand*{\bibfont}{\footnotesize}
\DefineBibliographyStrings{english}{references = {References}}

%% Include the adsurl field key into those that are recognized:
\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map{
      \step[fieldsource=adsurl,fieldtarget=iswc]
      \step[fieldsource=gbkurl,fieldtarget=iswc]
    }
  }
}

%% Set the color of the doi link to mymg (magenta) and the ads links
%% to mypurp (or purple):
\definecolor{mypurp}{cmyk}{0.75,1,0,0}
\newcommand{\doihref}[2]{\href{#1}{\color{magenta}{#2}}}
\newcommand{\adshref}[2]{\href{#1}{\color{mypurp}{#2}}}
\newcommand{\blackhref}[2]{\href{#1}{\color{black}{#2}}}

%% Define a format for the printtext commands in
%% DeclareBibliographyDriver to make links for the doi, ads link and
%% arxiv link:
\DeclareFieldFormat{doilink}{
  \iffieldundef{doi}{#1}{\doihref{http://dx.doi.org/\thefield{doi}}{#1}}}
\DeclareFieldFormat{adslink}{
    \iffieldundef{iswc}{#1}{\adshref{\thefield{iswc}}{#1}}}
\DeclareFieldFormat{arxivlink}{
  \iffieldundef{eprint}{#1}{\href{http://arxiv.org/abs/\thefield{eprint}}{#1}}}

\DeclareListFormat{doiforbook}{
  \iffieldundef{doi}{#1}{\doihref{http://dx.doi.org/\thefield{doi}}{#1}}}
\DeclareFieldFormat{googlebookslink}{
    \iffieldundef{iswc}{#1}{\adshref{\thefield{iswc}}{#1}}}

%% Set the formatting to make the last three values into the
%% appropriate link. Note that the % signs are necessary. Without
%% them, the items will be indented.
\DeclareBibliographyDriver{article}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \newunit%
  \ifdefined\makethesis\printtext{\usebibmacro{title}}\fi%
  \newunit%
  \printtext[doilink]{\usebibmacro{journal}}%
  \addcomma%
  \printtext[adslink]{\printfield{volume}}%
  \addcomma%
  \printtext[arxivlink]{\printfield{pages}}%
  \addperiod%
}

\DeclareBibliographyDriver{book}{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \usebibmacro{author/translator+others}%
  \newunit%
  \printtext{\usebibmacro{title}}%
  \addperiod%
  \addspace%
  \printlist[doiforbook]{publisher}%
  \addcomma%
  \addspace%
  \printfield[googlebookslink]{edition}%
  \printtext{ ed.}%
  \addperiod%
}

%% In order to have et al. instead of et al.,:
\renewcommand*{\nameyeardelim}{\addspace}


==> tex/src/preamble-maneage-default-style.tex <==
%% General paper's style settings.
%
%% This preamble can be completely ignored when including this TeX file in
%% another style. This is done because this LaTeX build is meant to be an
%% initial/internal phase or part of a larger effort, so it has a basic
%% style defined here as a preamble. To ignore it, uncomment or delete the
%% respective line in 'paper.tex'.
%
%% Copyright (C) 2019-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%
%% This file is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the
%% Free Software Foundation, either version 3 of the License, or (at your
%% option) any later version.
%
%% This file is distributed in the hope that it will be useful, but WITHOUT
%% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General Public License
%% for more details.
%
%% You should have received a copy of the GNU General Public License along
%% with this file.  If not, see <http://www.gnu.org/licenses/>.





%% Font.
\usepackage[T1]{fontenc}
\usepackage{newtxtext}
\usepackage{newtxmath}





%% Print size
\usepackage[a4paper, includeheadfoot, body={18.7cm, 24.5cm}]{geometry}





%% Set the distance between the columns if two columns:
\setlength{\columnsep}{0.75cm}





% To allow figures to take up more space on the top of the page:
\renewcommand{\topfraction}{.99}
\renewcommand{\bottomfraction}{.7}
\renewcommand{\textfraction}{.05}
\renewcommand{\floatpagefraction}{.99}
\renewcommand{\dbltopfraction}{.99}
\renewcommand{\dblfloatpagefraction}{.99}
\setcounter{topnumber}{1}
\setcounter{bottomnumber}{0}
\setcounter{totalnumber}{2}
\setcounter{dbltopnumber}{1}





%% To make the footnotes align:
\usepackage[hang]{footmisc}
\setlength\footnotemargin{10pt}





%For including time in the title:
\usepackage{datetime}





%% Define the abstract environment
\renewenvironment{abstract}
 {\vspace{-0.5cm}\small%
  \list{}{%
    \setlength{\leftmargin}{2cm}%
    \setlength{\rightmargin}{\leftmargin}%
  }%
  \item\relax}
 {\endlist}





%% To keep the main page's code clean.
\newcommand{\includeabstract}[1]{%
\twocolumn[%
  \begin{@twocolumnfalse}%
    \maketitle%
    \begin{abstract}%
    #1%
    \end{abstract}%
    \vspace{1cm}%
  \end{@twocolumnfalse}%
  ]%
}





%% Basic header style
%% ------------------
%
%% The steps below are to use the necessary LaTeX packages to get the demo
%% Maneage paper running with a reasonably looking, custom paper style. If
%% you are using a custom journal style, feel free to delete these.

%% General page header settings.
\usepackage{fancyhdr}
\pagestyle{fancy}
\lhead{\footnotesize{\scshape Draft paper}, {\footnotesize nnn:i (pp), Year Month day}}
\rhead{\scshape\footnotesize YOUR-NAME et al.}
\cfoot{\thepage}
\setlength{\voffset}{0.75cm}
\setlength{\headsep}{0.2cm}
\setlength{\footskip}{0.75cm}
\renewcommand{\headrulewidth}{0pt}

%% Specific style for first page.
\fancypagestyle{firststyle}
{
  \lhead{\footnotesize{\scshape Draft paper}, nnn:i (pp), YYYY Month day\\
  \scriptsize \textcopyright YYYY, Your name. All rights reserved.}
  \rhead{\footnotesize \footnotesize \today, \currenttime\\}
}

%To set the style of the titles:
\usepackage{titlesec}
\titleformat{\section}
  {\centering\normalfont\uppercase}
  {\thesection.}
  {0em}
  { }
\titleformat{\subsection}
  {\centering\normalsize\slshape}
  {\thesubsection.}
  {0em}
  { }
\titleformat{\subsubsection}
  {\centering\small\slshape}
  {\thesubsubsection.}
  {0em}
  { }

%% Title and author information
\usepackage{authblk}
\renewcommand\Authfont{\small\scshape}
\renewcommand\Affilfont{\footnotesize\normalfont}
\setlength{\affilsep}{0.2cm}


==> tex/src/references.tex <==
%% Non-software BibTeX entries. The software-specific BibTeX entries are
%% stored in a '*.tex' file under the 'tex/dependencies' directory.
%
%% Copyright (C) 2022-2025 Elham Saremi     <saremy.elham@gmail.com>
%% Copyright (C) 2018-2023 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{maneage,
       author = {{Akhlaghi}, Mohammad and {Infante-Sainz}, Raul and
         {Roukema}, Boudewijn F. and {Khellat}, Mohammadreza and
         {Valls-Gabaud}, David and {Baena-Galle}, Roberto},
        title = "{Toward Long-Term and Archivable Reproducibility}",
      journal = {CiSE},
     keywords = {Computer Science - Digital Libraries},
         year = 2021,
        month = may,
       volume = {23},
       number = {3},
        pages = {82-91},
          doi = {10.1109/MCSE.2021.3072860},
archivePrefix = {arXiv},
       eprint = {2006.03018},
 primaryClass = {cs.DL},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021CSE....23c..82A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{alliez19,
       author = {{Alliez}, Pierre and {Di Cosmo}, Roberto and {Guedj}, Benjamin and
         {Girault}, Alain and {Hacid}, Mohand-Said and {Legrand}, Arnaud and
         {Rougier}, Nicolas P.},
        title = "{Attributing and Referencing (Research) Software: Best Practices and Outlook from Inria}",
      journal = {CiSE},
       volume = {22},
         year = "2020",
        month = "Jan",
        pages = {39-52},
archivePrefix = {arXiv},
       eprint = {1905.11123},
 primaryClass = {cs.DL},
          doi = {10.1109/MCSE.2019.2949413},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190511123A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{infantesainz20,
       author = {{Infante-Sainz}, Ra{\'u}l and {Trujillo}, Ignacio and
         {Rom{\'a}n}, Javier},
        title = "{The Sloan Digital Sky Survey extended point spread functions}",
      journal = {MNRAS},
         year = 2020,
        month = feb,
       volume = {491},
       number = {4},
        pages = {5317-5329},
          doi = {10.1093/mnras/stz3111},
archivePrefix = {arXiv},
       eprint = {1911.01430},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.5317I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{infantesainz24b,
       author = {{Infante-Sainz}, Ra{\'u}l and {Akhlaghi}, Mohammad and {Eskandarlou}, Sepideh},
        title = "{Gnuastro: Measuring Radial Profiles from Images}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Astronomy software, Astronomical techniques, Astronomy data visualization, Broad band photometry, Open source software, 1855, 1684, 1968, 184, 1866, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = jan,
       volume = {8},
       number = {1},
          eid = {22},
        pages = {22},
          doi = {10.3847/2515-5172/ad1ee2},
archivePrefix = {arXiv},
       eprint = {2401.05303},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024RNAAS...8...22I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{infantesainz24a,
       author = {{Infante-Sainz}, Ra{\'u}l and {Akhlaghi}, Mohammad},
        title = "{Gnuastro: Visualizing the Full Dynamic Range in Color Images}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Astronomy software, Astronomy data visualization, Open source software, Low surface brightness galaxies, 1855, 1968, 1866, 940, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies, Computer Science - Computer Vision and Pattern Recognition},
         year = 2024,
        month = jan,
       volume = {8},
       number = {1},
          eid = {10},
        pages = {10},
          doi = {10.3847/2515-5172/ad1aae},
archivePrefix = {arXiv},
       eprint = {2401.03814},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024RNAAS...8...10I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Akhlaghi17,
       author = {{Akhlaghi}, M. and {Ichikawa}, T.},
        title = "{Noise-based Detection and Segmentation of Nebulous Signal: A review}",
    booktitle = {Astronomical Data Analysis Software and Systems XXV},
         year = 2017,
       editor = {{Lorente}, N.~P.~F. and {Shortridge}, K. and {Wayth}, R.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {512},
        month = dec,
        pages = {213},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ASPC..512..213A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@software{Akhlaghi18,
       author = {{Akhlaghi}, Mohammad},
        title = "{Gnuastro: GNU Astronomy Utilities}",
 howpublished = {Astrophysics Source Code Library, record ascl:1801.009},
         year = 2018,
        month = jan,
          eid = {ascl:1801.009},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ascl.soft01009A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Akhlaghi19a,
       author = {{Akhlaghi}, Mohammad},
        title = "{Carving out the low surface brightness universe with NoiseChisel}",
      journal = {IAU Symposium 335},
         year = 2019,
        month = sep,
          eid = {arXiv:1909.11230},
        pages = {arXiv:1909.11230},
archivePrefix = {arXiv},
       eprint = {1909.11230},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190911230A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Akhlaghi19b,
       author = {{Akhlaghi}, Mohammad},
        title = "{Separating Detection and Catalog Production}",
      journal = {ASPC},
         year = "2019",
        month = "Oct",
       volume = {521},
        pages = {299},
archivePrefix = {arXiv},
       eprint = {1611.06387},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ASPC..521..299A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Blanton07,
       author = {{Blanton}, Michael R. and {Roweis}, Sam},
        title = "{K-Corrections and Filter Transformations in the Ultraviolet, Optical, and Near-Infrared}",
      journal = {\aj},
     keywords = {galaxies: fundamental parameters, galaxies: photometry, galaxies: statistics, Astrophysics},
         year = 2007,
        month = feb,
       volume = {133},
       number = {2},
        pages = {734-754},
          doi = {10.1086/510127},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606170},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007AJ....133..734B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Cross12,
       author = {{Cross}, N.~J.~G. and {Collins}, R.~S. and {Mann}, R.~G. and {Read}, M.~A. and {Sutorius}, E.~T.~W. and {Blake}, R.~P. and {Holliman}, M. and {Hambly}, N.~C. and {Emerson}, J.~P. and {Lawrence}, A. and {Noddle}, K.~T.},
        title = "{The VISTA Science Archive}",
      journal = {\aap},
     keywords = {surveys, catalogs, astronomical databases: miscellaneous, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2012,
        month = dec,
       volume = {548},
          eid = {A119},
        pages = {A119},
          doi = {10.1051/0004-6361/201219505},
archivePrefix = {arXiv},
       eprint = {1210.2980},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...548A.119C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lang10,
       author = {{Lang}, Dustin and {Hogg}, David W. and {Mierle}, Keir and {Blanton}, Michael and {Roweis}, Sam},
        title = "{Astrometry.net: Blind Astrometric Calibration of Arbitrary Astronomical Images}",
      journal = {\aj},
     keywords = {astrometry, catalogs, instrumentation: miscellaneous, methods: data analysis, methods: statistical, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2010,
        month = may,
       volume = {139},
       number = {5},
        pages = {1782-1800},
          doi = {10.1088/0004-6256/139/5/1782},
archivePrefix = {arXiv},
       eprint = {0910.2233},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....139.1782L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gaia21,
       author = {{Gaia Collaboration},
       and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M. and {Creevey}, O.~L. and {Evans}, D.~W. and {Eyer}, L. and {Hutton}, A. and {Jansen}, F. and {Jordi}, C. and {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and {Mignard}, F. and {Panem}, C. and {Pourbaix}, D. and {Randich}, S. and {Sartoretti}, P. and {Soubiran}, C. and {Walton}, N.~A. and {Arenou}, F. and {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Cropper}, M. and {Drimmel}, R. and {Katz}, D. and {Lattanzi}, M.~G. and {van Leeuwen}, F. and {Bakker}, J. and {Cacciari}, C. and {Casta{\~n}eda}, J. and {De Angeli}, F. and {Ducourant}, C. and {Fabricius}, C. and {Fouesneau}, M. and {Fr{\'e}mat}, Y. and {Guerra}, R. and {Guerrier}, A. and {Guiraud}, J. and {Jean-Antoine Piccolo}, A. and {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and {Nicolas}, C. and {Nienartowicz}, K. and {Pailler}, F. and {Panuzzo}, P. and {Riclet}, F. and {Roux}, W. and {Seabroke}, G.~M. and {Sordo}, R. and {Tanga}, P. and {Th{\'e}venin}, F. and {Gracia-Abril}, G. and {Portell}, J. and {Teyssier}, D. and {Altmann}, M. and {Andrae}, R. and {Bellas-Velidis}, I. and {Benson}, K. and {Berthier}, J. and {Blomme}, R. and {Brugaletta}, E. and {Burgess}, P.~W. and {Busso}, G. and {Carry}, B. and {Cellino}, A. and {Cheek}, N. and {Clementini}, G. and {Damerdji}, Y. and {Davidson}, M. and {Delchambre}, L. and {Dell'Oro}, A. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and {Galluccio}, L. and {Garc{\'\i}a-Lario}, P. and {Garcia-Reinaldos}, M. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and {Gosset}, E. and {Haigron}, R. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and {Harrison}, D.~L. and {Hatzidimitriou}, D. and {Heiter}, U. and {Hern{\'a}ndez}, J. and {Hestroffer}, D. and {Hodgkin}, S.~T. and {Holl}, B. and {Jan{\ss}en}, K. and {Jevardat de Fombelle}, G. and {Jordan}, S. and {Krone-Martins}, A. and {Lanzafame}, A.~C. and {L{\"o}ffler}, W. and {Lorca}, A. and {Manteiga}, M. and {Marchal}, O. and {Marrese}, P.~M. and {Moitinho}, A. and {Mora}, A. and {Muinonen}, K. and {Osborne}, P. and {Pancino}, E. and {Pauwels}, T. and {Petit}, J. -M. and {Recio-Blanco}, A. and {Richards}, P.~J. and {Riello}, M. and {Rimoldini}, L. and {Robin}, A.~C. and {Roegiers}, T. and {Rybizki}, J. and {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Sozzetti}, A. and {Ulla}, A. and {Utrilla}, E. and {van Leeuwen}, M. and {van Reeven}, W. and {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and {Aerts}, C. and {Aguado}, J.~J. and {Ajaj}, M. and {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {{\'A}lvarez Cid-Fuentes}, J. and {Alves}, J. and {Anderson}, R.~I. and {Anglada Varela}, E. and {Antoja}, T. and {Audard}, M. and {Baines}, D. and {Baker}, S.~G. and {Balaguer-N{\'u}{\~n}ez}, L. and {Balbinot}, E. and {Balog}, Z. and {Barache}, C. and {Barbato}, D. and {Barros}, M. and {Barstow}, M.~A. and {Bartolom{\'e}}, S. and {Bassilana}, J. -L. and {Bauchet}, N. and {Baudesson-Stella}, A. and {Becciani}, U. and {Bellazzini}, M. and {Bernet}, M. and {Bertone}, S. and {Bianchi}, L. and {Blanco-Cuaresma}, S. and {Boch}, T. and {Bombrun}, A. and {Bossini}, D. and {Bouquillon}, S. and {Bragaglia}, A. and {Bramante}, L. and {Breedt}, E. and {Bressan}, A. and {Brouillet}, N. and {Bucciarelli}, B. and {Burlacu}, A. and {Busonero}, D. and {Butkevich}, A.~G. and {Buzzi}, R. and {Caffau}, E. and {Cancelliere}, R. and {C{\'a}novas}, H. and {Cantat-Gaudin}, T. and {Carballo}, R. and {Carlucci}, T. and {Carnerero}, M.~I. and {Carrasco}, J.~M. and {Casamiquela}, L. and {Castellani}, M. and {Castro-Ginard}, A. and {Castro Sampol}, P. and {Chaoul}, L. and {Charlot}, P. and {Chemin}, L. and {Chiavassa}, A. and {Cioni}, M. -R.~L. and {Comoretto}, G. and {Cooper}, W.~J. and {Cornez}, T. and {Cowell}, S. and {Crifo}, F. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and {Dapergolas}, A. and {David}, M. and {David}, P. and {de Laverny}, P. and {De Luise}, F. and {De March}, R. and {De Ridder}, J. and {de Souza}, R. and {de Teodoro}, P. and {de Torres}, A. and {del Peloso}, E.~F. and {del Pozo}, E. and {Delbo}, M. and {Delgado}, A. and {Delgado}, H.~E. and {Delisle}, J. -B. and {Di Matteo}, P. and {Diakite}, S. and {Diener}, C. and {Distefano}, E. and {Dolding}, C. and {Eappachen}, D. and {Edvardsson}, B. and {Enke}, H. and {Esquej}, P. and {Fabre}, C. and {Fabrizio}, M. and {Faigler}, S. and {Fedorets}, G. and {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Fouron}, C. and {Fragkoudi}, F. and {Fraile}, E. and {Franke}, F. and {Gai}, M. and {Garabato}, D. and {Garcia-Gutierrez}, A. and {Garc{\'\i}a-Torres}, M. and {Garofalo}, A. and {Gavras}, P. and {Gerlach}, E. and {Geyer}, R. and {Giacobbe}, P. and {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomel}, R. and {Gomez}, A. and {Gonzalez-Santamaria}, I. and {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Hauser}, M. and {Haywood}, M. and {Helmi}, A. and {Hidalgo}, S.~L. and {Hilger}, T. and {H{\l}adczuk}, N. and {Hobbs}, D. and {Holland}, G. and {Huckle}, H.~E. and {Jasniewicz}, G. and {Jonker}, P.~G. and {Juaristi Campillo}, J. and {Julbe}, F. and {Karbevska}, L. and {Kervella}, P. and {Khanna}, S. and {Kochoska}, A. and {Kontizas}, M. and {Kordopatis}, G. and {Korn}, A.~J. and {Kostrzewa-Rutkowska}, Z. and {Kruszy{\'n}ska}, K. and {Lambert}, S. and {Lanza}, A.~F. and {Lasne}, Y. and {Le Campion}, J. -F. and {Le Fustec}, Y. and {Lebreton}, Y. and {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and {Lecoeur-Taibi}, I. and {Liao}, S. and {Licata}, E. and {Lindstr{\o}m}, E.~P. and {Lister}, T.~A. and {Livanou}, E. and {Lobel}, A. and {Madrero Pardo}, P. and {Managau}, S. and {Mann}, R.~G. and {Marchant}, J.~M. and {Marconi}, M. and {Marcos Santos}, M.~M.~S. and {Marinoni}, S. and {Marocco}, F. and {Marshall}, D.~J. and {Martin Polo}, L. and {Mart{\'\i}n-Fleitas}, J.~M. and {Masip}, A. and {Massari}, D. and {Mastrobuono-Battisti}, A. and {Mazeh}, T. and {McMillan}, P.~J. and {Messina}, S. and {Michalik}, D. and {Millar}, N.~R. and {Mints}, A. and {Molina}, D. and {Molinaro}, R. and {Moln{\'a}r}, L. and {Montegriffo}, P. and {Mor}, R. and {Morbidelli}, R. and {Morel}, T. and {Morris}, D. and {Mulone}, A.~F. and {Munoz}, D. and {Muraveva}, T. and {Murphy}, C.~P. and {Musella}, I. and {Noval}, L. and {Ord{\'e}novic}, C. and {Orr{\`u}}, G. and {Osinde}, J. and {Pagani}, C. and {Pagano}, I. and {Palaversa}, L. and {Palicio}, P.~A. and {Panahi}, A. and {Pawlak}, M. and {Pe{\~n}alosa Esteller}, X. and {Penttil{\"a}}, A. and {Piersimoni}, A.~M. and {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poggio}, E. and {Poretti}, E. and {Poujoulet}, E. and {Pr{\v{s}}a}, A. and {Pulone}, L. and {Racero}, E. and {Ragaini}, S. and {Rainer}, M. and {Raiteri}, C.~M. and {Rambaux}, N. and {Ramos}, P. and {Ramos-Lerate}, M. and {Re Fiorentin}, P. and {Regibo}, S. and {Reyl{\'e}}, C. and {Ripepi}, V. and {Riva}, A. and {Rixon}, G. and {Robichon}, N. and {Robin}, C. and {Roelens}, M. and {Rohrbasser}, L. and {Romero-G{\'o}mez}, M. and {Rowell}, N. and {Royer}, F. and {Rybicki}, K.~A. and {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, A. and {Sahlmann}, J. and {Salgado}, J. and {Salguero}, E. and {Samaras}, N. and {Sanchez Gimenez}, V. and {Sanna}, N. and {Santove{\~n}a}, R. and {Sarasso}, M. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and {Segovia}, J.~C. and {S{\'e}gransan}, D. and {Semeux}, D. and {Shahaf}, S. and {Siddiqui}, H.~I. and {Siebert}, A. and {Siltala}, L. and {Slezak}, E. and {Smart}, R.~L. and {Solano}, E. and {Solitro}, F. and {Souami}, D. and {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and {Thuillot}, W. and {Tonello}, N. and {Torra}, F. and {Torra}, J. and {Turon}, C. and {Unger}, N. and {Vaillant}, M. and {van Dillen}, E. and {Vanel}, O. and {Vecchiato}, A. and {Viala}, Y. and {Vicente}, D. and {Voutsinas}, S. and {Weiler}, M. and {Wevers}, T. and {Wyrzykowski}, {\L}. and {Yoldas}, A. and {Yvard}, P. and {Zhao}, H. and {Zorec}, J. and {Zucker}, S. and {Zurbach}, C. and {Zwitter}, T.},
        title = "{Gaia Early Data Release 3. Summary of the contents and survey properties}",
      journal = {\aap},
     keywords = {catalogs, astrometry, parallaxes, proper motions, techniques: photometric, techniques: radial velocities, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {649},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/202039657},
archivePrefix = {arXiv},
       eprint = {2012.01533},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...649A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Cross12,
       author = {{Cross}, N.~J.~G. and {Collins}, R.~S. and {Mann}, R.~G. and {Read}, M.~A. and {Sutorius}, E.~T.~W. and {Blake}, R.~P. and {Holliman}, M. and {Hambly}, N.~C. and {Emerson}, J.~P. and {Lawrence}, A. and {Noddle}, K.~T.},
        title = "{The VISTA Science Archive}",
      journal = {\aap},
     keywords = {surveys, catalogs, astronomical databases: miscellaneous, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2012,
        month = dec,
       volume = {548},
          eid = {A119},
        pages = {A119},
          doi = {10.1051/0004-6361/201219505},
archivePrefix = {arXiv},
       eprint = {1210.2980},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...548A.119C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Maihara93,
       author = {{Maihara}, Toshinori and {Iwamuro}, Fumihide and {Yamashita}, Takuya and {Hall}, Donald N.~B. and {Cowie}, Lennox L. and {Tokunaga}, Alan T. and {Pickles}, Andrew},
        title = "{Observations of the OH Airglow Emission}",
      journal = {\pasp},
     keywords = {Airglow, Background Radiation, Hydroxyl Radicals, Spectral Bands, Spectral Emission, Infrared Astronomy, Line Spectra, Near Infrared Radiation, Geophysics, ATMOSPHERIC EFFECTS, LINE: IDENTIFICATION, TECHNIQUES: PHOTOMETRIC},
         year = 1993,
        month = sep,
       volume = {105},
        pages = {940},
          doi = {10.1086/133259},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993PASP..105..940M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Borlaff19,
       author = {{Borlaff}, Alejandro and {Trujillo}, Ignacio and {Rom{\'a}n}, Javier and {Beckman}, John E. and {Eliche-Moral}, M. Carmen and {Infante-S{\'a}inz}, Ra{\'u}l and {Lumbreras-Calle}, Alejandro and {de Almagro}, Rodrigo Takuro Sato Mart{\'\i}n and {G{\'o}mez-Guijarro}, Carlos and {Cebri{\'a}n}, Mar{\'\i}a and {Dorta}, Antonio and {Cardiel}, Nicol{\'a}s and {Akhlaghi}, Mohammad and {Mart{\'\i}nez-Lombilla}, Cristina},
        title = "{The missing light of the Hubble Ultra Deep Field}",
      journal = {\aap},
     keywords = {techniques: image processing, techniques: photometric, methods: observational, galaxies: evolution, galaxies: structure, galaxies: high-redshift, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jan,
       volume = {621},
          eid = {A133},
        pages = {A133},
          doi = {10.1051/0004-6361/201834312},
archivePrefix = {arXiv},
       eprint = {1810.00002},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...621A.133B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Brammer16,
       author = {{Brammer}, G.~B. and {Marchesini}, D. and {Labb{\'e}}, I. and {Spitler}, L. and {Lange-Vagle}, D. and {Barker}, E.~A. and {Tanaka}, M. and {Fontana}, A. and {Galametz}, A. and {Ferr{\'e}-Mateu}, A. and {Kodama}, T. and {Lundgren}, B. and {Martis}, N. and {Muzzin}, A. and {Stefanon}, M. and {Toft}, S. and {van der Wel}, A. and {Vulcani}, B. and {Whitaker}, K.~E.},
        title = "{Ultra-deep K-band Imaging of the Hubble Frontier Fields}",
      journal = {The Messenger},
         year = 2016,
        month = sep,
       volume = {165},
        pages = {34-37},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016Msngr.165...34B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Grosbol04,
       author = {{Grosb{\o}l}, P. and {Patsis}, P.~A. and {Pompei}, E.},
        title = "{Spiral galaxies observed in the near-infrared K band.  I. Data analysis and structural parameters}",
      journal = {\aap},
     keywords = {galaxies: photometry, galaxies: spiral, galaxies: structure, galaxies: fundamental parameters, infrared: galaxies},
         year = 2004,
        month = sep,
       volume = {423},
        pages = {849-859},
          doi = {10.1051/0004-6361:20035804},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...423..849G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Pisano11,
       author = {{Pisano}, D.~J. and {Barnes}, David G. and {Staveley-Smith}, Lister and {Gibson}, Brad K. and {Kilborn}, Virginia A. and {Freeman}, Ken C.},
        title = "{An H I Survey of Six Local Group Analogs. II. H I Properties of Group Galaxies}",
      journal = {\apjs},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: groups: general, galaxies: luminosity function, mass function, Local Group, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = dec,
       volume = {197},
       number = {2},
          eid = {28},
        pages = {28},
          doi = {10.1088/0067-0049/197/2/28},
archivePrefix = {arXiv},
       eprint = {1110.3431},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..197...28P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Mihos15,
       author = {{Mihos}, J. Christopher and {Durrell}, Patrick R. and {Ferrarese}, Laura and {Feldmeier}, John J. and {C{\^o}t{\'e}}, Patrick and {Peng}, Eric W. and {Harding}, Paul and {Liu}, Chengze and {Gwyn}, Stephen and {Cuillandre}, Jean-Charles},
        title = "{Galaxies at the Extremes: Ultra-diffuse Galaxies in the Virgo Cluster}",
      journal = {\apjl},
     keywords = {galaxies: clusters: individual: Virgo, galaxies: evolution, galaxies: fundamental parameters, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = aug,
       volume = {809},
       number = {2},
          eid = {L21},
        pages = {L21},
          doi = {10.1088/2041-8205/809/2/L21},
archivePrefix = {arXiv},
       eprint = {1507.02270},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...809L..21M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Mihos24,
       author = {{Mihos}, J. Christopher and {Durrell}, Patrick R. and {Watkins}, Aaron E. and {McGaugh}, Stacy S. and {Feldmeier}, John},
        title = "{BST1047+1156: A (Failing) Ultradiffuse Tidal Dwarf in the Leo I Group}",
      journal = {\apj},
     keywords = {Low surface brightness galaxies, Stellar populations, Galaxy evolution, Galaxy environments, Galaxy groups, 940, 1622, 594, 2029, 597, Astrophysics - Astrophysics of Galaxies},
         year = 2024,
        month = mar,
       volume = {964},
       number = {1},
          eid = {67},
        pages = {67},
          doi = {10.3847/1538-4357/ad1cef},
archivePrefix = {arXiv},
       eprint = {2401.03985},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJ...964...67M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{vanDokkum15,
       author = {{van Dokkum}, Pieter G. and {Abraham}, Roberto and {Merritt}, Allison and {Zhang}, Jielai and {Geha}, Marla and {Conroy}, Charlie},
        title = "{Forty-seven Milky Way-sized, Extremely Diffuse Galaxies in the Coma Cluster}",
      journal = {\apjl},
     keywords = {galaxies: clusters: individual: Coma, galaxies: evolution, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = jan,
       volume = {798},
       number = {2},
          eid = {L45},
        pages = {L45},
          doi = {10.1088/2041-8205/798/2/L45},
archivePrefix = {arXiv},
       eprint = {1410.8141},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798L..45V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Venhola17,
       author = {{Venhola}, Aku and {Peletier}, Reynier and {Laurikainen}, Eija and {Salo}, Heikki and {Lisker}, Thorsten and {Iodice}, Enrichetta and {Capaccioli}, Massimo and {Verdois Kleijn}, Gijs and {Valentijn}, Edwin and {Mieske}, Steffen and {Hilker}, Michael and {Wittmann}, Carolin and {van de Ven}, Glenn and {Grado}, Aniello and {Spavone}, Marilena and {Cantiello}, Michele and {Napolitano}, Nicola and {Paolillo}, Maurizio and {Falc{\'o}n-Barroso}, Jes{\'u}s},
        title = "{The Fornax Deep Survey with VST. III. Low surface brightness dwarfs and ultra diffuse galaxies in the center of the Fornax cluster}",
      journal = {\aap},
     keywords = {galaxies: dwarf, galaxies: photometry, galaxies: evolution, galaxies: clusters: individual: Fornax, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = dec,
       volume = {608},
          eid = {A142},
        pages = {A142},
          doi = {10.1051/0004-6361/201730696},
archivePrefix = {arXiv},
       eprint = {1710.04616},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...608A.142V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zaritsky19,
       author = {{Zaritsky}, Dennis and {Donnerstein}, Richard and {Dey}, Arjun and {Kadowaki}, Jennifer and {Zhang}, Huanian and {Karunakaran}, Ananthan and {Mart{\'\i}nez-Delgado}, David and {Rahman}, Mubdi and {Spekkens}, Kristine},
        title = "{Systematically Measuring Ultra-diffuse Galaxies (SMUDGes). I. Survey Description and First Results in the Coma Galaxy Cluster and Environs}",
      journal = {\apjs},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = jan,
       volume = {240},
       number = {1},
          eid = {1},
        pages = {1},
          doi = {10.3847/1538-4365/aaefe9},
archivePrefix = {arXiv},
       eprint = {1811.04098},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..240....1Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zaritsky22,
       author = {{Zaritsky}, Dennis and {Donnerstein}, Richard and {Karunakaran}, Ananthan and {Barbosa}, C.~E. and {Dey}, Arjun and {Kadowaki}, Jennifer and {Spekkens}, Kristine and {Zhang}, Huanian},
        title = "{Systematically Measuring Ultra-diffuse Galaxies (SMUDGes). III. The Southern SMUDGes Catalog}",
      journal = {\apjs},
     keywords = {Low surface brightness galaxies, Galaxy structure, 940, 622, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = aug,
       volume = {261},
       number = {2},
          eid = {11},
        pages = {11},
          doi = {10.3847/1538-4365/ac6ceb},
archivePrefix = {arXiv},
       eprint = {2205.02193},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJS..261...11Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zaritsky23,
       author = {{Zaritsky}, Dennis and {Donnerstein}, Richard and {Dey}, Arjun and {Karunakaran}, Ananthan and {Kadowaki}, Jennifer and {Khim}, Donghyeon J. and {Spekkens}, Kristine and {Zhang}, Huanian},
        title = "{Systematically Measuring Ultra-diffuse Galaxies (SMUDGes). V. The Complete SMUDGes Catalog and the Nature of Ultradiffuse Galaxies}",
      journal = {\apjs},
     keywords = {Galaxy formation, Galaxy evolution, Galaxy properties, Low surface brightness galaxies, 595, 594, 615, 940, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = aug,
       volume = {267},
       number = {2},
          eid = {27},
        pages = {27},
          doi = {10.3847/1538-4365/acdd71},
archivePrefix = {arXiv},
       eprint = {2306.01524},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJS..267...27Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{FliriTrujillo16,
       author = {{Fliri}, J{\"u}rgen and {Trujillo}, Ignacio},
        title = "{The IAC Stripe 82 Legacy Project: a wide-area survey for faint surface brightness astronomy}",
      journal = {\mnras},
     keywords = {atlases, catalogues, surveys, stars: general, galaxies: general, galaxies: interactions, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = feb,
       volume = {456},
       number = {2},
        pages = {1359-1373},
          doi = {10.1093/mnras/stv2686},
archivePrefix = {arXiv},
       eprint = {1603.04474},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.456.1359F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{TrujilloFliri16,
       author = {{Trujillo}, Ignacio and {Fliri}, J{\"u}ergen},
        title = "{Beyond 31 mag arcsec$^{-2}$: The Frontier of Low Surface Brightness Imaging with the Largest Optical Telescopes}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: halos, galaxies: photometry, galaxies: spiral, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = jun,
       volume = {823},
       number = {2},
          eid = {123},
        pages = {123},
          doi = {10.3847/0004-637X/823/2/123},
archivePrefix = {arXiv},
       eprint = {1510.04696},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...823..123T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{MontesTrujillo14,
       author = {{Montes}, Mireia and {Trujillo}, Ignacio},
        title = "{Intracluster Light at the Frontier: A2744}",
      journal = {\apj},
     keywords = {galaxies: clusters: individual: A2744, galaxies: evolution, galaxies: halos, galaxies: photometry, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = oct,
       volume = {794},
       number = {2},
          eid = {137},
        pages = {137},
          doi = {10.1088/0004-637X/794/2/137},
archivePrefix = {arXiv},
       eprint = {1405.2070},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...794..137M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Montes19,
       author = {{Montes}, Mireia},
        title = "{The intracluster light and its role in galaxy evolution in clusters}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = dec,
          eid = {arXiv:1912.01616},
        pages = {arXiv:1912.01616},
          doi = {10.48550/arXiv.1912.01616},
archivePrefix = {arXiv},
       eprint = {1912.01616},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv191201616M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{MontesTrujillo22,
       author = {{Montes}, Mireia and {Trujillo}, Ignacio},
        title = "{A New Era of Intracluster Light Studies with JWST}",
      journal = {\apjl},
     keywords = {James Webb Space Telescope, Galaxy clusters, Dark matter distribution, 2291, 584, 356, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2022,
        month = dec,
       volume = {940},
       number = {2},
          eid = {L51},
        pages = {L51},
          doi = {10.3847/2041-8213/ac98c5},
archivePrefix = {arXiv},
       eprint = {2209.00043},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...940L..51M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Mihos17,
       author = {{Mihos}, J. Christopher and {Harding}, Paul and {Feldmeier}, John J. and {Rudick}, Craig and {Janowiecki}, Steven and {Morrison}, Heather and {Slater}, Colin and {Watkins}, Aaron},
        title = "{The Burrell Schmidt Deep Virgo Survey: Tidal Debris, Galaxy Halos, and Diffuse Intracluster Light in the Virgo Cluster}",
      journal = {\apj},
     keywords = {galaxies: clusters: individual: Virgo, galaxies: individual: M87, M49, NGC 4365, galaxies: interactions, techniques: photometric, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jan,
       volume = {834},
       number = {1},
          eid = {16},
        pages = {16},
          doi = {10.3847/1538-4357/834/1/16},
archivePrefix = {arXiv},
       eprint = {1611.04435},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834...16M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Montes22,
       author = {{Montes}, Mireia},
        title = "{The faint light in groups and clusters of galaxies}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2022,
        month = mar,
       volume = {6},
        pages = {308-316},
          doi = {10.1038/s41550-022-01616-z},
archivePrefix = {arXiv},
       eprint = {2203.06199},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022NatAs...6..308M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{DeMaio18,
       author = {{DeMaio}, Tahlia and {Gonzalez}, Anthony H. and {Zabludoff}, Ann and {Zaritsky}, Dennis and {Connor}, Thomas and {Donahue}, Megan and {Mulchaey}, John S.},
        title = "{Lost but not forgotten: intracluster light in galaxy groups and clusters}",
      journal = {\mnras},
     keywords = {galaxies: clusters: general, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = mar,
       volume = {474},
       number = {3},
        pages = {3009-3031},
          doi = {10.1093/mnras/stx2946},
archivePrefix = {arXiv},
       eprint = {1710.11313},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.474.3009D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Contini21,
       author = {{Contini}, Emanuele},
        title = "{On the Origin and Evolution of the Intra-Cluster Light: A Brief Review of the Most Recent Developments}",
      journal = {Galaxies},
     keywords = {galaxy clusters, galaxy formation, galaxy evolution, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = aug,
       volume = {9},
       number = {3},
          eid = {60},
        pages = {60},
          doi = {10.3390/galaxies9030060},
archivePrefix = {arXiv},
       eprint = {2107.04180},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021Galax...9...60C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kluge20,
       author = {{Kluge}, M. and {Neureiter}, B. and {Riffeser}, A. and {Bender}, R. and {Goessl}, C. and {Hopp}, U. and {Schmidt}, M. and {Ries}, C. and {Brosch}, N.},
        title = "{Structure of Brightest Cluster Galaxies and Intracluster Light}",
      journal = {\apjs},
     keywords = {cD galaxies, Galaxy formation, Galaxy stellar halos, Surface photometry, Scaling relations, Brightest cluster galaxies, 209, 595, 598, 1670, 2031, 181, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = apr,
       volume = {247},
       number = {2},
          eid = {43},
        pages = {43},
          doi = {10.3847/1538-4365/ab733b},
archivePrefix = {arXiv},
       eprint = {1908.08544},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJS..247...43K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Ellien25,
       author = {{Ellien}, A. and {Montes}, M. and {Ahad}, S.~L. and {Dimauro}, P. and {Golden-Marx}, J.~B. and {Jimenez-Teja}, Y. and {Durret}, F. and {Bellhouse}, C. and {Diego}, J.~M. and {Bamford}, S.~P. and {Gonzalez}, A.~H. and {Hatch}, N.~A. and {Kluge}, M. and {Ragusa}, R. and {Slezak}, E. and {Cuillandre}, J. -C. and {Gavazzi}, R. and {Dole}, H. and {Mahler}, G. and {Congedo}, G. and {Saifollahi}, T. and {Aghanim}, N. and {Altieri}, B. and {Amara}, A. and {Andreon}, S. and {Auricchio}, N. and {Baccigalupi}, C. and {Baldi}, M. and {Balestra}, A. and {Bardelli}, S. and {Basset}, A. and {Battaglia}, P. and {Biviano}, A. and {Bonchi}, A. and {Bonino}, D. and {Branchini}, E. and {Brescia}, M. and {Brinchmann}, J. and {Caillat}, A. and {Camera}, S. and {Capobianco}, V. and {Carbone}, C. and {Cardone}, V.~F. and {Carretero}, J. and {Casas}, S. and {Castellano}, M. and {Castignani}, G. and {Cavuoti}, S. and {Cimatti}, A. and {Colodro-Conde}, C. and {Conselice}, C.~J. and {Conversi}, L. and {Copin}, Y. and {Courbin}, F. and {Courtois}, H.~M. and {Cropper}, M. and {Da Silva}, A. and {Degaudenzi}, H. and {De Lucia}, G. and {Di Giorgio}, A.~M. and {Dinis}, J. and {Dubath}, F. and {Duncan}, C.~A.~J. and {Dupac}, X. and {Dusini}, S. and {Farina}, M. and {Faustini}, F. and {Ferriol}, S. and {Fotopoulou}, S. and {Frailis}, M. and {Franceschi}, E. and {Galeotta}, S. and {George}, K. and {Gillis}, B. and {Giocoli}, C. and {G{\'o}mez-Alvarez}, P. and {Grazian}, A. and {Grupp}, F. and {Guzzo}, L. and {Haugan}, S.~V.~H. and {Hoar}, J. and {Hoekstra}, H. and {Holmes}, W. and {Hormuth}, F. and {Hornstrup}, A. and {Hudelot}, P. and {Jahnke}, K. and {Jhabvala}, M. and {Joachimi}, B. and {Keih{\"a}nen}, E. and {Kermiche}, S. and {Kiessling}, A. and {Kubik}, B. and {Kuijken}, K. and {K{\"u}mmel}, M. and {Kunz}, M. and {Kurki-Suonio}, H. and {Laureijs}, R. and {Le Mignant}, D. and {Ligori}, S. and {Lilje}, P.~B. and {Lindholm}, V. and {Lloro}, I. and {Mainetti}, G. and {Maino}, D. and {Maiorano}, E. and {Mansutti}, O. and {Marcin}, S. and {Marggraf}, O. and {Markovic}, K. and {Martinelli}, M. and {Martinet}, N. and {Marulli}, F. and {Massey}, R. and {Maurogordato}, S. and {Medinaceli}, E. and {Mei}, S. and {Melchior}, M. and {Mellier}, Y. and {Meneghetti}, M. and {Merlin}, E. and {Meylan}, G. and {Mora}, A. and {Moresco}, M. and {Moscardini}, L. and {Nakajima}, R. and {Neissner}, C. and {Nichol}, R.~C. and {Niemi}, S. -M. and {Nightingale}, J.~W. and {Padilla}, C. and {Paltani}, S. and {Pasian}, F. and {Pedersen}, K. and {Percival}, W.~J. and {Pettorino}, V. and {Pires}, S. and {Polenta}, G. and {Poncet}, M. and {Popa}, L.~A. and {Pozzetti}, L. and {Raison}, F. and {Rebolo}, R. and {Renzi}, A. and {Rhodes}, J. and {Riccio}, G. and {Romelli}, E. and {Roncarelli}, M. and {Rossetti}, E. and {Saglia}, R. and {Sakr}, Z. and {Sapone}, D. and {Sartoris}, B. and {Scaramella}, R. and {Schirmer}, M. and {Schneider}, P. and {Schrabback}, T. and {Secroun}, A. and {Sefusatti}, E. and {Seidel}, G. and {Seiffert}, M. and {Serrano}, S. and {Sirignano}, C. and {Sirri}, G. and {Stanco}, L. and {Starck}, J. -L. and {Steinwagner}, J. and {Tallada-Cresp{\'\i}}, P. and {Taylor}, A.~N. and {Teplitz}, H.~I. and {Tereno}, I. and {Toledo-Moreo}, R. and {Torradeflot}, F. and {Tsyganov}, A. and {Tutusaus}, I. and {Valenziano}, L. and {Vassallo}, T. and {Verdoes Kleijn}, G. and {Veropalumbo}, A. and {Wang}, Y. and {Weller}, J. and {Williams}, O.~R. and {Zucca}, E. and {Bolzonella}, M. and {Burigana}, C. and {Scottez}, V.},
        title = "{Euclid: Early Release Observations: The intracluster light of Abell 2390}",
      journal = {\aap},
     keywords = {galaxies: clusters: general, galaxies: clusters: intracluster medium, galaxies: clusters: individual: Abell 2390, Astrophysics of Galaxies},
         year = 2025,
        month = jun,
       volume = {698},
          eid = {A134},
        pages = {A134},
          doi = {10.1051/0004-6361/202554460},
archivePrefix = {arXiv},
       eprint = {2503.07484},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025A&A...698A.134E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hilton21,
       author = {{Hilton}, M. and {Sif{\'o}n}, C. and {Naess}, S. and {Madhavacheril}, M. and {Oguri}, M. and {Rozo}, E. and {Rykoff}, E. and {Abbott}, T.~M.~C. and {Adhikari}, S. and {Aguena}, M. and {Aiola}, S. and {Allam}, S. and {Amodeo}, S. and {Amon}, A. and {Annis}, J. and {Ansarinejad}, B. and {Aros-Bunster}, C. and {Austermann}, J.~E. and {Avila}, S. and {Bacon}, D. and {Battaglia}, N. and {Beall}, J.~A. and {Becker}, D.~T. and {Bernstein}, G.~M. and {Bertin}, E. and {Bhandarkar}, T. and {Bhargava}, S. and {Bond}, J.~R. and {Brooks}, D. and {Burke}, D.~L. and {Calabrese}, E. and {Carrasco Kind}, M. and {Carretero}, J. and {Choi}, S.~K. and {Choi}, A. and {Conselice}, C. and {da Costa}, L.~N. and {Costanzi}, M. and {Crichton}, D. and {Crowley}, K.~T. and {D{\"u}nner}, R. and {Denison}, E.~V. and {Devlin}, M.~J. and {Dicker}, S.~R. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Duff}, S.~M. and {Duivenvoorden}, A.~J. and {Dunkley}, J. and {Everett}, S. and {Ferraro}, S. and {Ferrero}, I. and {Fert{\'e}}, A. and {Flaugher}, B. and {Frieman}, J. and {Gallardo}, P.~A. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giles}, P. and {Golec}, J.~E. and {Gralla}, M.~B. and {Grandis}, S. and {Gruen}, D. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Han}, D. and {Hartley}, W.~G. and {Hasselfield}, M. and {Hill}, J.~C. and {Hilton}, G.~C. and {Hincks}, A.~D. and {Hinton}, S.~R. and {Ho}, S. -P.~P. and {Honscheid}, K. and {Hoyle}, B. and {Hubmayr}, J. and {Huffenberger}, K.~M. and {Hughes}, J.~P. and {Jaelani}, A.~T. and {Jain}, B. and {James}, D.~J. and {Jeltema}, T. and {Kent}, S. and {Knowles}, K. and {Koopman}, B.~J. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, Y. -T. and {Lokken}, M. and {Loubser}, S.~I. and {MacCrann}, N. and {Maia}, M.~A.~G. and {Marriage}, T.~A. and {Martin}, J. and {McMahon}, J. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Miyatake}, H. and {Moodley}, K. and {Morgan}, R. and {Mroczkowski}, T. and {Nati}, F. and {Newburgh}, L.~B. and {Niemack}, M.~D. and {Nishizawa}, A.~J. and {Ogando}, R.~L.~C. and {Orlowski-Scherer}, J. and {Page}, L.~A. and {Palmese}, A. and {Partridge}, B. and {Paz-Chinch{\'o}n}, F. and {Phakathi}, P. and {Plazas}, A.~A. and {Robertson}, N.~C. and {Romer}, A.~K. and {Carnero Rosell}, A. and {Salatino}, M. and {Sanchez}, E. and {Schaan}, E. and {Schillaci}, A. and {Sehgal}, N. and {Serrano}, S. and {Shin}, T. and {Simon}, S.~M. and {Smith}, M. and {Soares-Santos}, M. and {Spergel}, D.~N. and {Staggs}, S.~T. and {Storer}, E.~R. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Trac}, H. and {Ullom}, J.~N. and {Vale}, L.~R. and {Van Lanen}, J. and {Vavagiakis}, E.~M. and {De Vicente}, J. and {Wilkinson}, R.~D. and {Wollack}, E.~J. and {Xu}, Z. and {Zhang}, Y.},
        title = "{The Atacama Cosmology Telescope: A Catalog of >4000 Sunyaev-Zel{\textquoteright}dovich Galaxy Clusters}",
      journal = {\apjs},
     keywords = {Galaxy clusters, Cosmology, Large-scale structure of the universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = mar,
       volume = {253},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.3847/1538-4365/abd023},
archivePrefix = {arXiv},
       eprint = {2009.11043},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJS..253....3H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Jarvis13,
       author = {{Jarvis}, Matt J. and {Bonfield}, D.~G. and {Bruce}, V.~A. and {Geach}, J.~E. and {McAlpine}, K. and {McLure}, R.~J. and {Gonz{\'a}lez-Solares}, E. and {Irwin}, M. and {Lewis}, J. and {Yoldas}, A. Kupcu and {Andreon}, S. and {Cross}, N.~J.~G. and {Emerson}, J.~P. and {Dalton}, G. and {Dunlop}, J.~S. and {Hodgkin}, S.~T. and {Le}, F{\`e}vre O. and {Karouzos}, M. and {Meisenheimer}, K. and {Oliver}, S. and {Rawlings}, S. and {Simpson}, C. and {Smail}, I. and {Smith}, D.~J.~B. and {Sullivan}, M. and {Sutherland}, W. and {White}, S.~V. and {Zwart}, J.~T.~L.},
        title = "{The VISTA Deep Extragalactic Observations (VIDEO) survey}",
      journal = {\mnras},
     keywords = {astronomical data bases: miscellaneous, surveys, large-scale structure of Universe, galaxies: general, galaxies: high redshift, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = jan,
       volume = {428},
       number = {2},
        pages = {1281-1295},
          doi = {10.1093/mnras/sts118},
archivePrefix = {arXiv},
       eprint = {1206.4263},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.428.1281J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Irwin04,
       author = {{Irwin}, Mike J. and {Lewis}, Jim and {Hodgkin}, Simon and {Bunclark}, Peter and {Evans}, Dafydd and {McMahon}, Richard and {Emerson}, James P. and {Stewart}, Malcolm and {Beard}, Steven},
        title = "{VISTA data flow system: pipeline processing for WFCAM and VISTA}",
    booktitle = {Optimizing Scientific Return for Astronomy through Information Technologies},
         year = 2004,
       editor = {{Quinn}, Peter J. and {Bridger}, Alan},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {5493},
        month = sep,
        pages = {411-422},
          doi = {10.1117/12.551449},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004SPIE.5493..411I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{McGaugh14,
       author = {{McGaugh}, Stacy S. and {Schombert}, James M.},
        title = "{Color-Mass-to-light-ratio Relations for Disk Galaxies}",
      journal = {\aj},
     keywords = {galaxies: evolution, galaxies: fundamental parameters, galaxies: photometry, galaxies: stellar content, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = nov,
       volume = {148},
       number = {5},
          eid = {77},
        pages = {77},
          doi = {10.1088/0004-6256/148/5/77},
archivePrefix = {arXiv},
       eprint = {1407.1839},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014AJ....148...77M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Caputi05,
       author = {{Caputi}, K.~I. and {Dunlop}, J.~S. and {McLure}, R.~J. and {Roche}, N.~D.},
        title = "{The evolution of K$_{s}$-selected galaxies in the GOODS/CDFS deep ISAAC field}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: high-redshift, galaxies: luminosity function, mass function, Astrophysics},
         year = 2005,
        month = aug,
       volume = {361},
       number = {2},
        pages = {607-622},
          doi = {10.1111/j.1365-2966.2005.09222.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0408373},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.361..607C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kochanek01,
       author = {{Kochanek}, C.~S. and {Pahre}, M.~A. and {Falco}, E.~E. and {Huchra}, J.~P. and {Mader}, J. and {Jarrett}, T.~H. and {Chester}, T. and {Cutri}, R. and {Schneider}, S.~E.},
        title = "{The K-Band Galaxy Luminosity Function}",
      journal = {\apj},
     keywords = {Cosmology: Observations, Galaxies: Distances and Redshifts, Galaxies: Luminosity Function, Mass Function, Surveys, Astrophysics},
         year = 2001,
        month = oct,
       volume = {560},
       number = {2},
        pages = {566-579},
          doi = {10.1086/322488},
archivePrefix = {arXiv},
       eprint = {astro-ph/0011456},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...560..566K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Sureshkumar21,
       author = {{Sureshkumar}, U. and {Durkalec}, A. and {Pollo}, A. and {Bilicki}, M. and {Loveday}, J. and {Farrow}, D.~J. and {Holwerda}, B.~W. and {Hopkins}, A.~M. and {Liske}, J. and {Pimbblet}, K.~A. and {Taylor}, E.~N. and {Wright}, A.~H.},
        title = "{Galaxy and Mass Assembly (GAMA). Tracing galaxy environment using the marked correlation function}",
      journal = {\aap},
     keywords = {large-scale structure of Universe, galaxies: statistics, galaxies: formation, galaxies: evolution, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = sep,
       volume = {653},
          eid = {A35},
        pages = {A35},
          doi = {10.1051/0004-6361/202140500},
archivePrefix = {arXiv},
       eprint = {2102.04177},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...653A..35S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Furusawa11,
       author = {{Furusawa}, Junko and {Sekiguchi}, Kazuhiro and {Takata}, Tadafumi and {Furusawa}, Hisanori and {Shimasaku}, Kazuhiro and {Simpson}, Chris and {Akiyama}, Masayuki},
        title = "{The Mass-dependent Clustering History of K-selected Galaxies at z < 4 in the SXDS/UDS Field}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: luminosity function, mass function, large-scale structure of universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = feb,
       volume = {727},
       number = {2},
          eid = {111},
        pages = {111},
          doi = {10.1088/0004-637X/727/2/111},
archivePrefix = {arXiv},
       eprint = {1101.1566},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...727..111F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Deng20,
       author = {{Deng}, Xin-Fa and {Wen}, Xiao-Qing and {Xin}, Yong and {Qi}, Xiao-Ping and {Ding}, Ying-Ping},
        title = "{K-band luminosity-density relation at fixed parameters or for different galaxy families}",
      journal = {Open Physics},
     keywords = {fundamental parameters of galaxies, statistic of galaxy, distance and redshifts},
         year = 2020,
        month = jul,
       volume = {18},
       number = {1},
          eid = {16},
        pages = {16},
          doi = {10.1515/phys-2020-0016},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020OPhy...18...16D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bell03,
       author = {{Bell}, Eric F. and {McIntosh}, Daniel H. and {Katz}, Neal and {Weinberg}, Martin D.},
        title = "{The Optical and Near-Infrared Properties of Galaxies. I. Luminosity and Stellar Mass Functions}",
      journal = {\apjs},
     keywords = {Galaxies: Evolution, Galaxies: General, Galaxies: Luminosity Function, Mass Function, Galaxies: Stellar Content, Astrophysics},
         year = 2003,
        month = dec,
       volume = {149},
       number = {2},
        pages = {289-312},
          doi = {10.1086/378847},
archivePrefix = {arXiv},
       eprint = {astro-ph/0302543},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJS..149..289B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Drory04,
       author = {{Drory}, N. and {Bender}, R. and {Feulner}, G. and {Hopp}, U. and {Maraston}, C. and {Snigula}, J. and {Hill}, G.~J.},
        title = "{The Munich Near-Infrared Cluster Survey (MUNICS). VI. The Stellar Masses of K-Band-selected Field Galaxies to z\raisebox{-0.5ex}\textasciitilde1.2}",
      journal = {\apj},
     keywords = {Cosmology: Observations, Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Luminosity Function, Mass Function, Surveys, Astrophysics},
         year = 2004,
        month = jun,
       volume = {608},
       number = {2},
        pages = {742-751},
          doi = {10.1086/420781},
archivePrefix = {arXiv},
       eprint = {astro-ph/0403041},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...608..742D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Dannerbauer22,
       author = {{Dannerbauer}, H. and {Carnero}, A. and {Cross}, N. and {Gutierrez}, C.~M.},
        title = "{Exploring the Universe via the Wide, Deep Near-infrared Imaging ESO Public Survey SHARKS}",
      journal = {The Messenger},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jun,
       volume = {187},
        pages = {12-15},
          doi = {10.18727/0722-6691/5265},
archivePrefix = {arXiv},
       eprint = {2212.09471},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022Msngr.187...12D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{McMahon13,
       author = {{McMahon}, R.~G. and {Banerji}, M. and {Gonzalez}, E. and {Koposov}, S.~E. and {Bejar}, V.~J. and {Lodieu}, N. and {Rebolo}, R. and {VHS Collaboration}},
        title = "{First Scientific Results from the VISTA Hemisphere Survey (VHS)}",
      journal = {The Messenger},
         year = 2013,
        month = dec,
       volume = {154},
        pages = {35-37},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013Msngr.154...35M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Edge13,
       author = {{Edge}, A. and {Sutherland}, W. and {Kuijken}, K. and {Driver}, S. and {McMahon}, R. and {Eales}, S. and {Emerson}, J.~P.},
        title = "{The VISTA Kilo-degree Infrared Galaxy (VIKING) Survey: Bridging the Gap between Low and High Redshift}",
      journal = {The Messenger},
         year = 2013,
        month = dec,
       volume = {154},
        pages = {32-34},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013Msngr.154...32E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Emerson06,
       author = {{Emerson}, J. and {McPherson}, A. and {Sutherland}, W.},
        title = "{Visible and Infrared Survey Telescope for Astronomy: Progress Report}",
      journal = {The Messenger},
         year = 2006,
        month = dec,
       volume = {126},
        pages = {41-42},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006Msngr.126...41E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Emerson04,
       author = {{Emerson}, James P. and {Irwin}, Mike J. and {Lewis}, Jim and {Hodgkin}, Simon and {Evans}, Dafydd and {Bunclark}, Peter and {McMahon}, Richard and {Hambly}, Nigel C. and {Mann}, Robert G. and {Bond}, Ian and {Sutorius}, Eckhard and {Read}, Michael and {Williams}, Peredur and {Lawrence}, Andrew and {Stewart}, Malcolm},
        title = "{VISTA data flow system: overview}",
    booktitle = {Optimizing Scientific Return for Astronomy through Information Technologies},
         year = 2004,
       editor = {{Quinn}, Peter J. and {Bridger}, Alan},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {5493},
        month = sep,
        pages = {401-410},
          doi = {10.1117/12.551582},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004SPIE.5493..401E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Roman21,
       author = {{Rom{\'a}n}, Javier and {Castilla}, Aida and {Pascual-Granado}, Javier},
        title = "{Discovery and analysis of low-surface-brightness galaxies in the environment of NGC 1052}",
      journal = {\aap},
     keywords = {galaxies: dwarf, galaxies: photometry, galaxies: groups: individual: NGC 1052, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = dec,
       volume = {656},
          eid = {A44},
        pages = {A44},
          doi = {10.1051/0004-6361/202142161},
archivePrefix = {arXiv},
       eprint = {2110.09527},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...656A..44R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Hambly08,
       author = {{Hambly}, N.~C. and {Collins}, R.~S. and {Cross}, N.~J.~G. and {Mann}, R.~G. and {Read}, M.~A. and {Sutorius}, E.~T.~W. and {Bond}, I. and {Bryant}, J. and {Emerson}, J.~P. and {Lawrence}, A. and {Rimoldini}, L. and {Stewart}, J.~M. and {Williams}, P.~M. and {Adamson}, A. and {Hirst}, P. and {Dye}, S. and {Warren}, S.~J.},
        title = "{The WFCAM Science Archive}",
      journal = {\mnras},
     keywords = {astronomical data bases: miscellaneous, surveys, stars: general, galaxies: general, cosmology: observations, infrared: general, Astrophysics},
         year = 2008,
        month = feb,
       volume = {384},
       number = {2},
        pages = {637-662},
          doi = {10.1111/j.1365-2966.2007.12700.x},
archivePrefix = {arXiv},
       eprint = {0711.3593},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.384..637H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lawrence07,
       author = {{Lawrence}, A. and {Warren}, S.~J. and {Almaini}, O. and {Edge}, A.~C. and {Hambly}, N.~C. and {Jameson}, R.~F. and {Lucas}, P. and {Casali}, M. and {Adamson}, A. and {Dye}, S. and {Emerson}, J.~P. and {Foucaud}, S. and {Hewett}, P. and {Hirst}, P. and {Hodgkin}, S.~T. and {Irwin}, M.~J. and {Lodieu}, N. and {McMahon}, R.~G. and {Simpson}, C. and {Smail}, I. and {Mortlock}, D. and {Folger}, M.},
        title = "{The UKIRT Infrared Deep Sky Survey (UKIDSS)}",
      journal = {\mnras},
     keywords = {surveys, infrared: general, Astrophysics},
         year = 2007,
        month = aug,
       volume = {379},
       number = {4},
        pages = {1599-1617},
          doi = {10.1111/j.1365-2966.2007.12040.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0604426},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.379.1599L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Minniti10,
       author = {{Minniti}, D. and {Lucas}, P.~W. and {Emerson}, J.~P. and {Saito}, R.~K. and {Hempel}, M. and {Pietrukowicz}, P. and {Ahumada}, A.~V. and {Alonso}, M.~V. and {Alonso-Garcia}, J. and {Arias}, J.~I. and {Bandyopadhyay}, R.~M. and {Barb{\'a}}, R.~H. and {Barbuy}, B. and {Bedin}, L.~R. and {Bica}, E. and {Borissova}, J. and {Bronfman}, L. and {Carraro}, G. and {Catelan}, M. and {Clari{\'a}}, J.~J. and {Cross}, N. and {de Grijs}, R. and {D{\'e}k{\'a}ny}, I. and {Drew}, J.~E. and {Fari{\~n}a}, C. and {Feinstein}, C. and {Fern{\'a}ndez Laj{\'u}s}, E. and {Gamen}, R.~C. and {Geisler}, D. and {Gieren}, W. and {Goldman}, B. and {Gonzalez}, O.~A. and {Gunthardt}, G. and {Gurovich}, S. and {Hambly}, N.~C. and {Irwin}, M.~J. and {Ivanov}, V.~D. and {Jord{\'a}n}, A. and {Kerins}, E. and {Kinemuchi}, K. and {Kurtev}, R. and {L{\'o}pez-Corredoira}, M. and {Maccarone}, T. and {Masetti}, N. and {Merlo}, D. and {Messineo}, M. and {Mirabel}, I.~F. and {Monaco}, L. and {Morelli}, L. and {Padilla}, N. and {Palma}, T. and {Parisi}, M.~C. and {Pignata}, G. and {Rejkuba}, M. and {Roman-Lopes}, A. and {Sale}, S.~E. and {Schreiber}, M.~R. and {Schr{\"o}der}, A.~C. and {Smith}, M. and {}, Jr., L. Sodr{\'e} and {Soto}, M. and {Tamura}, M. and {Tappert}, C. and {Thompson}, M.~A. and {Toledo}, I. and {Zoccali}, M. and {Pietrzynski}, G.},
        title = "{VISTA Variables in the Via Lactea (VVV): The public ESO near-IR variability survey of the Milky Way}",
      journal = {\na},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = jul,
       volume = {15},
       number = {5},
        pages = {433-443},
          doi = {10.1016/j.newast.2009.12.002},
archivePrefix = {arXiv},
       eprint = {0912.1056},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010NewA...15..433M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Cioni11,
       author = {{Cioni}, M. -R.~L. and {Clementini}, G. and {Girardi}, L. and {Guandalini}, R. and {Gullieuszik}, M. and {Miszalski}, B. and {Moretti}, M. -I. and {Ripepi}, V. and {Rubele}, S. and {Bagheri}, G. and {Bekki}, K. and {Cross}, N. and {de Blok}, W.~J.~G. and {de Grijs}, R. and {Emerson}, J.~P. and {Evans}, C.~J. and {Gibson}, B. and {Gonzales-Solares}, E. and {Groenewegen}, M.~A.~T. and {Irwin}, M. and {Ivanov}, V.~D. and {Lewis}, J. and {Marconi}, M. and {Marquette}, J. -B. and {Mastropietro}, C. and {Moore}, B. and {Napiwotzki}, R. and {Naylor}, T. and {Oliveira}, J.~M. and {Read}, M. and {Sutorius}, E. and {van Loon}, J. Th. and {Wilkinson}, M.~I. and {Wood}, P.~R.},
        title = "{The VMC survey. I. Strategy and first data}",
      journal = {\aap},
     keywords = {magellanic clouds, infrared: stars, stars: variables: Cepheids, stars: variables: RR Lyrae, Hertzsprung-Russell and C-M diagrams, survey, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = mar,
       volume = {527},
          eid = {A116},
        pages = {A116},
          doi = {10.1051/0004-6361/201016137},
archivePrefix = {arXiv},
       eprint = {1012.5193},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...527A.116C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Honig17,
       author = {{H{\"o}nig}, S.~F. and {Watson}, D. and {Kishimoto}, M. and {Gandhi}, P. and {Goad}, M. and {Horne}, K. and {Shankar}, F. and {Banerji}, M. and {Boulderstone}, B. and {Jarvis}, M. and {Smith}, M. and {Sullivan}, M.},
        title = "{Cosmology with AGN dust time lags-simulating the new VEILS survey}",
      journal = {\mnras},
     keywords = {galaxies: active, distance scale, infrared: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jan,
       volume = {464},
       number = {2},
        pages = {1693-1703},
          doi = {10.1093/mnras/stw2484},
archivePrefix = {arXiv},
       eprint = {1609.09091},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.464.1693H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{McCracken12,
       author = {{McCracken}, H.~J. and {Milvang-Jensen}, B. and {Dunlop}, J. and {Franx}, M. and {Fynbo}, J.~P.~U. and {Le F{\`e}vre}, O. and {Holt}, J. and {Caputi}, K.~I. and {Goranova}, Y. and {Buitrago}, F. and {Emerson}, J.~P. and {Freudling}, W. and {Hudelot}, P. and {L{\'o}pez-Sanjuan}, C. and {Magnard}, F. and {Mellier}, Y. and {M{\o}ller}, P. and {Nilsson}, K.~K. and {Sutherland}, W. and {Tasca}, L. and {Zabl}, J.},
        title = "{UltraVISTA: a new ultra-deep near-infrared survey in COSMOS}",
      journal = {\aap},
     keywords = {surveys, galaxies: general, galaxies: high-redshift, cosmology: observations, large-scale structure of Universe, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2012,
        month = aug,
       volume = {544},
          eid = {A156},
        pages = {A156},
          doi = {10.1051/0004-6361/201219507},
archivePrefix = {arXiv},
       eprint = {1204.6586},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...544A.156M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Meingast23,
       author = {{Meingast}, S. and {Alves}, J. and {Bouy}, H. and {VISIONS Collaboration}},
        title = "{The VISTA Star Formation Atlas (VISIONS)}",
      journal = {The Messenger},
         year = 2023,
        month = sep,
       volume = {191},
        pages = {18-22},
          doi = {10.18727/0722-6691/5336},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023Msngr.191...18M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Bertin06,
       author = {{Bertin}, E.},
        title = "{Automatic Astrometric and Photometric Calibration with SCAMP}",
    booktitle = {Astronomical Data Analysis Software and Systems XV},
         year = 2006,
       editor = {{Gabriel}, C. and {Arviset}, C. and {Ponz}, D. and {Enrique}, S.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {351},
        month = jul,
        pages = {112},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..351..112B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bertin96,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {\aaps},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = 1996,
        month = jun,
       volume = {117},
        pages = {393-404},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Cuby00,
       author = {{Cuby}, J.~G. and {Lidman}, C. and {Moutou}, C.},
        title = "{ISAAC: 18 Months of Paranal Science Operations}",
      journal = {The Messenger},
         year = 2000,
        month = sep,
       volume = {101},
        pages = {2-8},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000Msngr.101....2C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Eskandarlou23,
       author = {{Eskandarlou}, Sepideh and {Akhlaghi}, Mohammad and {Infante-Sainz}, Ra{\'u}l and {Saremi}, Elham and {Raji}, Samane and {Sharbaf}, Zahra and {Golini}, Giulia and {Ghaffari}, Zohreh and {Knapen}, Johan H.},
        title = "{Gnuastro: Estimating the Zero-point Magnitude in Astronomical Imaging}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Flux calibration, Astronomy software, Open source software, Astronomical techniques, 544, 1855, 1866, 1684, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2023,
        month = dec,
       volume = {7},
       number = {12},
          eid = {269},
        pages = {269},
          doi = {10.3847/2515-5172/ad14f4},
archivePrefix = {arXiv},
       eprint = {2312.04263},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023RNAAS...7..269E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Trujillo21,
       author = {{Trujillo}, Ignacio and {D'Onofrio}, Mauro and {Zaritsky}, Dennis and {Madrigal-Aguado}, Alberto and {Chamba}, Nushkia and {Golini}, Giulia and {Akhlaghi}, Mohammad and {Sharbaf}, Zahra and {Infante-Sainz}, Ra{\'u}l and {Rom{\'a}n}, Javier and {Morales-Socorro}, Carlos and {Sand}, David J. and {Martin}, Garreth},
        title = "{Introducing the LBT Imaging of Galactic Halos and Tidal Structures (LIGHTS) survey. A preview of the low surface brightness Universe to be unveiled by LSST}",
      journal = {\aap},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: halos, galaxies: photometry, galaxies: structure, dark matter, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = oct,
       volume = {654},
          eid = {A40},
        pages = {A40},
          doi = {10.1051/0004-6361/202141603},
archivePrefix = {arXiv},
       eprint = {2109.07478},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...654A..40T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Euclid25,
       author = {{Euclid Collaboration} and {Jahnke}, K. and {Gillard}, W. and {Schirmer}, M. and {Ealet}, A. and {Maciaszek}, T. and {Prieto}, E. and {Barbier}, R. and {Bonoli}, C. and {Corcione}, L. and {Dusini}, S. and {Grupp}, F. and {Hormuth}, F. and {Ligori}, S. and {Martin}, L. and {Morgante}, G. and {Padilla}, C. and {Toledo-Moreo}, R. and {Trifoglio}, M. and {Valenziano}, L. and {Bender}, R. and {Castander}, F.~J. and {Garilli}, B. and {Lilje}, P.~B. and {Rix}, H. -W. and {Andersen}, M.~I. and {Auricchio}, N. and {Balestra}, A. and {Barriere}, J. -C. and {Battaglia}, P. and {Berthe}, M. and {Bodendorf}, C. and {Boenke}, T. and {Bon}, W. and {Bonnefoi}, A. and {Caillat}, A. and {Capobianco}, V. and {Carle}, M. and {Casas}, R. and {Cho}, H. and {Costille}, A. and {Ducret}, F. and {Ferriol}, S. and {Franceschi}, E. and {Gimenez}, J. -L. and {Holmes}, W. and {Hornstrup}, A. and {Jhabvala}, M. and {Kohley}, R. and {Kubik}, B. and {Laureijs}, R. and {Le Mignant}, D. and {Lloro}, I. and {Medinaceli}, E. and {Mellier}, Y. and {Polenta}, G. and {Racca}, G.~D. and {Renzi}, A. and {Salvignol}, J. -C. and {Secroun}, A. and {Seidel}, G. and {Seiffert}, M. and {Sirignano}, C. and {Sirri}, G. and {Strada}, P. and {Smadja}, G. and {Stanco}, L. and {Wachter}, S. and {Anselmi}, S. and {Borsato}, E. and {Caillat}, L. and {Cogato}, F. and {Colodro-Conde}, C. and {Crouzet}, P. -E. and {Conforti}, V. and {D'Alessandro}, M. and {Copin}, Y. and {Cuillandre}, J. -C. and {Davies}, J.~E. and {Davini}, S. and {Derosa}, A. and {Diaz}, J.~J. and {Di Domizio}, S. and {Di Ferdinando}, D. and {Farinelli}, R. and {Ferrari}, A.~G. and {Fornari}, F. and {Gabarra}, L. and {Garcia}, R. and {Gutierrez}, C.~M. and {Giacomini}, F. and {Lagier}, P. and {Gianotti}, F. and {Krause}, O. and {Madrid}, F. and {Laudisio}, F. and {Macias-Perez}, J. and {Naletto}, G. and {Niclas}, M. and {Marpaud}, J. and {Mauri}, N. and {da Silva}, R. and {Passalacqua}, F. and {Paterson}, K. and {Patrizii}, L. and {Risso}, I. and {Solheim}, B.~G.~B. and {Scodeggio}, M. and {Stassi}, P. and {Steinwagner}, J. and {Tenti}, M. and {Testera}, G. and {Travaglini}, R. and {Tosi}, S. and {Troja}, A. and {Tubio}, O. and {Valieri}, C. and {Vescovi}, C. and {Ventura}, S. and {Aghanim}, N. and {Altieri}, B. and {Amara}, A. and {Amiaux}, J. and {Andreon}, S. and {Appleton}, P.~N. and {Aussel}, H. and {Baccigalupi}, C. and {Baldi}, M. and {Bardelli}, S. and {Basset}, A. and {Bonchi}, A. and {Bonino}, D. and {Branchini}, E. and {Brescia}, M. and {Brinchmann}, J. and {Camera}, S. and {Carbone}, C. and {Cardone}, V.~F. and {Carretero}, J. and {Casas}, S. and {Castellano}, M. and {Castignani}, G. and {Cavuoti}, S. and {Chabaud}, P. -Y. and {Cimatti}, A. and {Congedo}, G. and {Conselice}, C.~J. and {Conversi}, L. and {Courbin}, F. and {Courtois}, H.~M. and {Crocce}, M. and {Cropper}, M. and {Cuby}, J. -G. and {Da Silva}, A. and {Degaudenzi}, H. and {De Lucia}, G. and {Di Giorgio}, A.~M. and {Dinis}, J. and {Douspis}, M. and {Dubath}, F. and {Duncan}, C.~A.~J. and {Dupac}, X. and {Fabricius}, M. and {Farina}, M. and {Farrens}, S. and {Faustini}, F. and {Fosalba}, P. and {Fotopoulou}, S. and {Fourmanoit}, N. and {Frailis}, M. and {Franzetti}, P. and {Galeotta}, S. and {George}, K. and {Gillis}, B. and {Giocoli}, C. and {G{\'o}mez-Alvarez}, P. and {Granett}, B.~R. and {Grazian}, A. and {Guzzo}, L. and {Hailey}, M. and {Haugan}, S.~V.~H. and {Hoar}, J. and {Hoekstra}, H. and {Hook}, I. and {Hudelot}, P. and {Ili{\'c}}, S. and {Joachimi}, B. and {Keih{\"a}nen}, E. and {Kermiche}, S. and {Kiessling}, A. and {Kilbinger}, M. and {Kitching}, T. and {K{\"u}mmel}, M. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lahav}, O. and {Liebing}, P. and {Lindholm}, V. and {Lorenzo Alvarez}, J. and {Mainetti}, G.},
        title = "{Euclid: III. The NISP Instrument}",
      journal = {\aap},
     keywords = {instrumentation: photometers, instrumentation: spectrographs, space vehicles: instruments, surveys, cosmology: observations, infrared: general, Instrumentation and Methods for Astrophysics, Cosmology and Nongalactic Astrophysics, Astrophysics of Galaxies},
         year = 2025,
        month = may,
       volume = {697},
          eid = {A3},
        pages = {A3},
          doi = {10.1051/0004-6361/202450786},
archivePrefix = {arXiv},
       eprint = {2405.13493},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025A&A...697A...3E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Conroy13,
       author = {{Conroy}, Charlie},
        title = "{Modeling the Panchromatic Spectral Energy Distributions of Galaxies}",
      journal = {\araa},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = aug,
       volume = {51},
       number = {1},
        pages = {393-455},
          doi = {10.1146/annurev-astro-082812-141017},
archivePrefix = {arXiv},
       eprint = {1301.7095},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ARA&A..51..393C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Zibetti09,
       author = {{Zibetti}, Stefano and {Charlot}, St{\'e}phane and {Rix}, Hans-Walter},
        title = "{Resolved stellar mass maps of galaxies - I. Method and implications for global mass estimates}",
      journal = {\mnras},
     keywords = {techniques: image processing, techniques: photometric, galaxies: fundamental parameters, galaxies: general, galaxies: photometry, galaxies: stellar content, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2009,
        month = dec,
       volume = {400},
       number = {3},
        pages = {1181-1198},
          doi = {10.1111/j.1365-2966.2009.15528.x},
archivePrefix = {arXiv},
       eprint = {0904.4252},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.400.1181Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kendall08,
       author = {{Kendall}, S. and {Kennicutt}, R.~C. and {Clarke}, C. and {Thornley}, M.~D.},
        title = "{Tracing spiral density waves in M81}",
      journal = {\mnras},
     keywords = {galaxies: individual: M81, galaxies: spiral, galaxies: structure, infrared: galaxies, Astrophysics},
         year = 2008,
        month = jul,
       volume = {387},
       number = {3},
        pages = {1007-1020},
          doi = {10.1111/j.1365-2966.2008.13327.x},
archivePrefix = {arXiv},
       eprint = {0804.2380},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.387.1007K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Euclid22,
       author = {{Euclid Collaboration} and {Moneti}, A. and {McCracken}, H.~J. and {Shuntov}, M. and {Kauffmann}, O.~B. and {Capak}, P. and {Davidzon}, I. and {Ilbert}, O. and {Scarlata}, C. and {Toft}, S. and {Weaver}, J. and {Chary}, R. and {Cuby}, J. and {Faisst}, A.~L. and {Masters}, D.~C. and {McPartland}, C. and {Mobasher}, B. and {Sanders}, D.~B. and {Scaramella}, R. and {Stern}, D. and {Szapudi}, I. and {Teplitz}, H. and {Zalesky}, L. and {Amara}, A. and {Auricchio}, N. and {Bodendorf}, C. and {Bonino}, D. and {Branchini}, E. and {Brau-Nogue}, S. and {Brescia}, M. and {Brinchmann}, J. and {Capobianco}, V. and {Carbone}, C. and {Carretero}, J. and {Castander}, F.~J. and {Castellano}, M. and {Cavuoti}, S. and {Cimatti}, A. and {Cledassou}, R. and {Congedo}, G. and {Conselice}, C.~J. and {Conversi}, L. and {Copin}, Y. and {Corcione}, L. and {Costille}, A. and {Cropper}, M. and {Da Silva}, A. and {Degaudenzi}, H. and {Douspis}, M. and {Dubath}, F. and {Duncan}, C.~A.~J. and {Dupac}, X. and {Dusini}, S. and {Farrens}, S. and {Ferriol}, S. and {Fosalba}, P. and {Frailis}, M. and {Franceschi}, E. and {Fumana}, M. and {Garilli}, B. and {Gillis}, B. and {Giocoli}, C. and {Granett}, B.~R. and {Grazian}, A. and {Grupp}, F. and {Haugan}, S.~V.~H. and {Hoekstra}, H. and {Holmes}, W. and {Hormuth}, F. and {Hudelot}, P. and {Jahnke}, K. and {Kermiche}, S. and {Kiessling}, A. and {Kilbinger}, M. and {Kitching}, T. and {Kohley}, R. and {K{\"u}mmel}, M. and {Kunz}, M. and {Kurki-Suonio}, H. and {Ligori}, S. and {Lilje}, P.~B. and {Lloro}, I. and {Maiorano}, E. and {Mansutti}, O. and {Marggraf}, O. and {Markovic}, K. and {Marulli}, F. and {Massey}, R. and {Maurogordato}, S. and {Meneghetti}, M. and {Merlin}, E. and {Meylan}, G. and {Moresco}, M. and {Moscardini}, L. and {Munari}, E. and {Niemi}, S.~M. and {Padilla}, C. and {Paltani}, S. and {Pasian}, F. and {Pedersen}, K. and {Pires}, S. and {Poncet}, M. and {Popa}, L. and {Pozzetti}, L. and {Raison}, F. and {Rebolo}, R. and {Rhodes}, J. and {Rix}, H. and {Roncarelli}, M. and {Rossetti}, E. and {Saglia}, R. and {Schneider}, P. and {Secroun}, A. and {Seidel}, G. and {Serrano}, S. and {Sirignano}, C. and {Sirri}, G. and {Stanco}, L. and {Tallada-Cresp{\'\i}}, P. and {Taylor}, A.~N. and {Tereno}, I. and {Toledo-Moreo}, R. and {Torradeflot}, F. and {Wang}, Y. and {Welikala}, N. and {Weller}, J. and {Zamorani}, G. and {Zoubian}, J. and {Andreon}, S. and {Bardelli}, S. and {Camera}, S. and {Graci{\'a}-Carpio}, J. and {Medinaceli}, E. and {Mei}, S. and {Polenta}, G. and {Romelli}, E. and {Sureau}, F. and {Tenti}, M. and {Vassallo}, T. and {Zacchei}, A. and {Zucca}, E. and {Baccigalupi}, C. and {Balaguera-Antol{\'\i}nez}, A. and {Bernardeau}, F. and {Biviano}, A. and {Bolzonella}, M. and {Bozzo}, E. and {Burigana}, C. and {Cabanac}, R. and {Cappi}, A. and {Carvalho}, C.~S. and {Casas}, S. and {Castignani}, G. and {Colodro-Conde}, C. and {Coupon}, J. and {Courtois}, H.~M. and {Di Ferdinando}, D. and {Farina}, M. and {Finelli}, F. and {Flose-Reimberg}, P. and {Fotopoulou}, S. and {Galeotta}, S. and {Ganga}, K. and {Garcia-Bellido}, J. and {Gaztanaga}, E. and {Gozaliasl}, G. and {Hook}, I. and {Joachimi}, B. and {Kansal}, V. and {Keihanen}, E. and {Kirkpatrick}, C.~C. and {Lindholm}, V. and {Mainetti}, G. and {Maino}, D. and {Maoli}, R. and {Martinelli}, M. and {Martinet}, N. and {Maturi}, M. and {Metcalf}, R.~B. and {Morgante}, G. and {Morisset}, N. and {Nucita}, A. and {Patrizii}, L. and {Potter}, D. and {Renzi}, A. and {Riccio}, G. and {S{\'a}nchez}, A.~G. and {Sapone}, D. and {Schirmer}, M. and {Schultheis}, M. and {Scottez}, V. and {Sefusatti}, E. and {Teyssier}, R. and {Tubio}, O. and {Tutusaus}, I. and {Valiviita}, J. and {Viel}, M. and {Hildebrandt}, H.},
        title = "{Euclid preparation. XVII. Cosmic Dawn Survey: Spitzer Space Telescope observations of the Euclid deep fields and calibration fields}",
      journal = {\aap},
     keywords = {cosmology: observations, large-scale structure of Universe, dark energy, dark matter, Galaxy: formation, surveys, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2022,
        month = feb,
       volume = {658},
          eid = {A126},
        pages = {A126},
          doi = {10.1051/0004-6361/202142361},
archivePrefix = {arXiv},
       eprint = {2110.13928},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...658A.126E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Sutherland15,
       author = {{Sutherland}, Will and {Emerson}, Jim and {Dalton}, Gavin and {Atad-Ettedgui}, Eli and {Beard}, Steven and {Bennett}, Richard and {Bezawada}, Naidu and {Born}, Andrew and {Caldwell}, Martin and {Clark}, Paul and {Craig}, Simon and {Henry}, David and {Jeffers}, Paul and {Little}, Bryan and {McPherson}, Alistair and {Murray}, John and {Stewart}, Malcolm and {Stobie}, Brian and {Terrett}, David and {Ward}, Kim and {Whalley}, Martin and {Woodhouse}, Guy},
        title = "{The Visible and Infrared Survey Telescope for Astronomy (VISTA): Design, technical overview, and performance}",
      journal = {\aap},
     keywords = {telescopes, instrumentation: photometers, instrumentation: miscellaneous, instrumentation: detectors, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = mar,
       volume = {575},
          eid = {A25},
        pages = {A25},
          doi = {10.1051/0004-6361/201424973},
archivePrefix = {arXiv},
       eprint = {1409.4780},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...575A..25S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gris24,
       author = {{Gris}, Philippe and {Awan}, Humna and {Becker}, Matthew R. and {Lin}, Huan and {Gawiser}, Eric and {Jha}, Saurabh W. and {The LSST Dark Energy Science Collaboration}},
        title = "{A Cohesive Deep Drilling Field Strategy for LSST Cosmology}",
      journal = {\apjs},
     keywords = {Cosmology, Cosmological parameters, Dark energy, Type Ia supernovae, 343, 339, 351, 1728, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2024,
        month = dec,
       volume = {275},
       number = {2},
          eid = {21},
        pages = {21},
          doi = {10.3847/1538-4365/ad79f5},
archivePrefix = {arXiv},
       eprint = {2405.10781},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024ApJS..275...21G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Euclid23,
       author = {{Euclid Collaboration} and {Gabarra}, L. and {Mancini}, C. and {Rodriguez Mu{\~n}oz}, L. and {Rodighiero}, G. and {Sirignano}, C. and {Scodeggio}, M. and {Talia}, M. and {Dusini}, S. and {Gillard}, W. and {Granett}, B.~R. and {Maiorano}, E. and {Moresco}, M. and {Paganin}, L. and {Palazzi}, E. and {Pozzetti}, L. and {Renzi}, A. and {Rossetti}, E. and {Vergani}, D. and {Allevato}, V. and {Bisigello}, L. and {Castignani}, G. and {De Caro}, B. and {Fumana}, M. and {Ganga}, K. and {Garilli}, B. and {Hirschmann}, M. and {La Franca}, F. and {Laigle}, C. and {Passalacqua}, F. and {Schirmer}, M. and {Stanco}, L. and {Troja}, A. and {Yung}, L.~Y.~A. and {Zamorani}, G. and {Zoubian}, J. and {Anselmi}, S. and {Oppizzi}, F. and {Verza}, G. and {Aghanim}, N. and {Amara}, A. and {Auricchio}, N. and {Baldi}, M. and {Bender}, R. and {Bodendorf}, C. and {Bonino}, D. and {Branchini}, E. and {Brescia}, M. and {Brinchmann}, J. and {Camera}, S. and {Capobianco}, V. and {Carbone}, C. and {Carretero}, J. and {Castander}, F.~J. and {Castellano}, M. and {Cavuoti}, S. and {Cledassou}, R. and {Congedo}, G. and {Conselice}, C.~J. and {Conversi}, L. and {Copin}, Y. and {Corcione}, L. and {Costille}, A. and {Courbin}, F. and {Da Silva}, A. and {Degaudenzi}, H. and {Dinis}, J. and {Dubath}, F. and {Dupac}, X. and {Ealet}, A. and {Farrens}, S. and {Ferriol}, S. and {Frailis}, M. and {Franceschi}, E. and {Franzetti}, P. and {Galeotta}, S. and {Gillis}, B. and {Giocoli}, C. and {Grazian}, A. and {Grupp}, F. and {Guzzo}, L. and {Holmes}, W. and {Hornstrup}, A. and {Hudelot}, P. and {Jahnke}, K. and {K{\"u}mmel}, M. and {Kermiche}, S. and {Kiessling}, A. and {Kilbinger}, M. and {Kitching}, T. and {Kohley}, R. and {Kubik}, B. and {Kunz}, M. and {Kurki-Suonio}, H. and {Ligori}, S. and {Lilje}, P.~B. and {Lloro}, I. and {Mansutti}, O. and {Marggraf}, O. and {Markovic}, K. and {Marulli}, F. and {Massey}, R. and {Maurogordato}, S. and {Mei}, S. and {Meneghetti}, M. and {Meylan}, G. and {Moscardini}, L. and {Munari}, E. and {Nichol}, R.~C. and {Niemi}, S. -M. and {Nightingale}, J. and {Padilla}, C. and {Paltani}, S. and {Pasian}, F. and {Pedersen}, K. and {Percival}, W.~J. and {Pettorino}, V. and {Polenta}, G. and {Poncet}, M. and {Raison}, F. and {Rhodes}, J. and {Riccio}, G. and {Romelli}, E. and {Roncarelli}, M. and {Saglia}, R. and {Sapone}, D. and {Schneider}, P. and {Secroun}, A. and {Seidel}, G. and {Serrano}, S. and {Sirri}, G. and {Surace}, C. and {Tallada-Cresp{\'\i}}, P. and {Tavagnacco}, D. and {Taylor}, A.~N. and {Tereno}, I. and {Toledo-Moreo}, R. and {Torradeflot}, F. and {Trifoglio}, M. and {Tutusaus}, I. and {Valentijn}, E.~A. and {Valenziano}, L. and {Vassallo}, T. and {Wang}, Y. and {Weller}, J. and {Zacchei}, A. and {Andreon}, S. and {Aussel}, H. and {Bardelli}, S. and {Bolzonella}, M. and {Boucaud}, A. and {Bozzo}, E. and {Colodro-Conde}, C. and {Di Ferdinando}, D. and {Farina}, M. and {Graci{\'a}-Carpio}, J. and {Keih{\"a}nen}, E. and {Lindholm}, V. and {Maino}, D. and {Mauri}, N. and {Mellier}, Y. and {Neissner}, C. and {Scottez}, V. and {Tenti}, M. and {Zucca}, E. and {Akrami}, Y. and {Baccigalupi}, C. and {Ballardini}, M. and {Bernardeau}, F. and {Biviano}, A. and {Borlaff}, A.~S. and {Borsato}, E. and {Burigana}, C. and {Cabanac}, R. and {Cappi}, A. and {Carvalho}, C.~S. and {Casas}, S. and {Castro}, T. and {Chambers}, K. and {Cooray}, A.~R. and {Coupon}, J. and {Courtois}, H.~M. and {Davini}, S. and {de la Torre}, S. and {De Lucia}, G. and {Desprez}, G. and {Dole}, H. and {Escartin}, J.~A. and {Escoffier}, S. and {Ferrero}, I. and {Finelli}, F. and {Fotopoulou}, S. and {Garcia-Bellido}, J. and {George}, K. and {Giacomini}, F. and {Gozaliasl}, G. and {Hildebrandt}, H. and {Hook}, I. and {Ilbert}, O. and {Jimenez Mu{\~n}oz}, A.},
        title = "{Euclid preparation. XXX. Performance assessment of the NISP red grism through spectroscopic simulations for the wide and deep surveys}",
      journal = {\aap},
     keywords = {surveys, Galaxy: evolution, galaxies: formation, galaxies: star formation, techniques: spectroscopic, instrumentation: detectors, Astrophysics - Astrophysics of Galaxies},
         year = 2023,
        month = aug,
       volume = {676},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/202346177},
archivePrefix = {arXiv},
       eprint = {2302.09372},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023A&A...676A..34E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Trinh13,
       author = {{Trinh}, Christopher Q. and {Ellis}, Simon C. and {Bland-Hawthorn}, Joss and {Horton}, Anthony J. and {Lawrence}, Jon S. and {Leon-Saval}, Sergio G.},
        title = "{The nature of the near-infrared interline sky background using fibre Bragg grating OH suppression}",
      journal = {\mnras},
     keywords = {atmospheric effects, instrumentation: miscellaneous, instrumentation: spectrographs, infrared: general, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2013,
        month = jul,
       volume = {432},
       number = {4},
        pages = {3262-3277},
          doi = {10.1093/mnras/stt677},
archivePrefix = {arXiv},
       eprint = {1301.0326},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.432.3262T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Buta15,
       author = {{Buta}, Ronald J. and {Sheth}, Kartik and {Athanassoula}, E. and {Bosma}, A. and {Knapen}, Johan H. and {Laurikainen}, Eija and {Salo}, Heikki and {Elmegreen}, Debra and {Ho}, Luis C. and {Zaritsky}, Dennis and {Courtois}, Helene and {Hinz}, Joannah L. and {Mu{\~n}oz-Mateos}, Juan-Carlos and {Kim}, Taehyun and {Regan}, Michael W. and {Gadotti}, Dimitri A. and {Gil de Paz}, Armando and {Laine}, Jarkko and {Men{\'e}ndez-Delmestre}, Kar{\'\i}n and {Comer{\'o}n}, S{\'e}bastien and {Erroz Ferrer}, Santiago and {Seibert}, Mark and {Mizusawa}, Trisha and {Holwerda}, Benne and {Madore}, Barry F.},
        title = "{A Classical Morphological Analysis of Galaxies in the Spitzer Survey of Stellar Structure in Galaxies (S4G)}",
      journal = {\apjs},
     keywords = {atlases, galaxies: elliptical and lenticular, galaxies: irregular, galaxies: spiral, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = apr,
       volume = {217},
       number = {2},
          eid = {32},
        pages = {32},
          doi = {10.1088/0067-0049/217/2/32},
archivePrefix = {arXiv},
       eprint = {1501.00454},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJS..217...32B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Schneider25,
       author = {{Schneider}, Adam C. and {Vrba}, Frederick J. and {Bruursema}, Justice and {Munn}, Jeffrey A. and {Irwin}, Mike and {Read}, Mike and {Varricatt}, Watson and {Kerr}, Tom and {Hodapp}, Klaus and {Dye}, Simon and {Williams}, Stephen J. and {Cenko}, Andrew T. and {Tilleman}, Trudy M. and {Murison}, Marc A. and {Rothberg}, Barry and {Dahm}, Scott and {Dorland}, Bryan and {Lawrence}, Andy and {Chambers}, Kenneth C.},
        title = "{The Second and Third Data Releases from the UKIRT Hemisphere Survey}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics of Galaxies, Instrumentation and Methods for Astrophysics, Solar and Stellar Astrophysics},
         year = 2025,
        month = jun,
          eid = {arXiv:2506.14621},
        pages = {arXiv:2506.14621},
          doi = {10.48550/arXiv.2506.14621},
archivePrefix = {arXiv},
       eprint = {2506.14621},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025arXiv250614621S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Conselice18,
       author = {{Conselice}, Christopher J.},
        title = "{Ultra-diffuse Galaxies Are a Subset of Cluster Dwarf Elliptical/Spheroidal Galaxies}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = mar,
       volume = {2},
       number = {1},
          eid = {43},
        pages = {43},
          doi = {10.3847/2515-5172/aab7f6},
archivePrefix = {arXiv},
       eprint = {1803.06927},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018RNAAS...2...43C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Sandage84,
       author = {{Sandage}, A. and {Binggeli}, B.},
        title = "{Studies of the Virgo cluster. III. A classification system and an illustrated Atlas of Virgo cluster dwarf galaxies.}",
      journal = {\aj},
     keywords = {Astronomical Catalogs, Dwarf Galaxies, Galactic Clusters, Virgo Galactic Cluster, Astronomical Photography, Luminosity, Spiral Galaxies, Astrophysics},
         year = 1984,
        month = jul,
       volume = {89},
        pages = {919-931},
          doi = {10.1086/113588},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984AJ.....89..919S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Impey88,
       author = {{Impey}, Chris and {Bothun}, Greg and {Malin}, David},
        title = "{Virgo Dwarfs: New Light on Faint Galaxies}",
      journal = {\apj},
     keywords = {Dwarf Galaxies, Faint Objects, Virgo Galactic Cluster, Astronomical Photometry, Brightness, Centimeter Waves, Hydrogen Atoms, Luminosity, Magnitude, Radio Galaxies, Red Shift, Spiral Galaxies, Astrophysics, GALAXIES: CLUSTERING, GALAXIES: PHOTOMETRY, GALAXIES: REDSHIFTS, GALAXIES: STELLAR CONTENT, GALAXIES: STRUCTURE, RADIO SOURCES: GALAXIES, RADIO SOURCES: 21 CM RADIATION},
         year = 1988,
        month = jul,
       volume = {330},
        pages = {634},
          doi = {10.1086/166500},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988ApJ...330..634I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Caldwell87,
       author = {{Caldwell}, Nelson and {Bothun}, Gregory D.},
        title = "{Dwarf Elliptical Galaxies in the Fornax Cluster. II. Their Structure and Stellar Populations}",
      journal = {\aj},
     keywords = {Dwarf Galaxies, Elliptical Galaxies, Galactic Clusters, Star Distribution, Astronomical Photometry, Charge Coupled Devices, Color, Distance, Galactic Nuclei, Virgo Galactic Cluster, Astrophysics, GALAXIES: GENERAL, GALAXIES: CLUSTERING},
         year = 1987,
        month = nov,
       volume = {94},
        pages = {1126},
          doi = {10.1086/114550},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987AJ.....94.1126C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> tex/src/temp2.tex <==
\def\imageWidth{2.0cm}
\def\imageHeight{2.0cm}
\def\distance{0.15cm}
\foreach \row in {0,...,6} {
  \foreach \col in {0,...,5} {
    \pgfmathtruncatemacro\index{5*\row + \col}
    \pgfmathsetmacro\imageIndex{\imageArray[\index]}
    \node[anchor=north west,inner sep=0,outer sep=0] at (\col*\imageWidth+\col*\distance,-\row*\imageHeight-\row*\distance)
         {\includegraphics[width=\imageWidth,height=\imageHeight]{\imageIndex}};
  }
}
\end{tikzpicture}
%\caption{42 PDF Images in a 6x7 grid}
\end{figure}
\end{document}


==> tex/src/temp3.tex <==
\def\imageWidth{2.0cm}
\def\imageHeight{2.0cm}
\def\distance{0.15cm}
\foreach \row in {0,...,3} {
  \foreach \col in {0,...,3} {
    \pgfmathtruncatemacro\index{4*\col + \row}
    \pgfmathsetmacro\imageIndex{\imageArray[\index]}
    \node[anchor=north west,inner sep=0,outer sep=0] at (\col*\imageWidth+\col*\distance,-\row*\imageHeight-\row*\distance)
         {\includegraphics[width=\imageWidth,height=\imageHeight]{\imageIndex}};
  }
}
\end{tikzpicture}
%\caption{16 PDF Images in a 4x4 grid}
\end{figure}
\end{document}

